Why are deep nets reversible: A simple theory, with implications for training

Generative models for deep learning are promising both to improve understanding of the model, and yield training methods requiring fewer labeled samples. Recent works use generative model approaches to produce the deep net's input given the value of a hidden layer several levels above. However, there is no accompanying "proof of correctness" for the generative model, showing that the feedforward deep net is the correct inference method for recovering the hidden layer given the input. Furthermore, these models are complicated. The current paper takes a more theoretical tack. It presents a very simple generative model for RELU deep nets, with the following characteristics: (i) The generative model is just the reverse of the feedforward net: if the forward transformation at a layer is $A$ then the reverse transformation is $A^T$. (This can be seen as an explanation of the old weight tying idea for denoising autoencoders.) (ii) Its correctness can be proven under a clean theoretical assumption: the edge weights in real-life deep nets behave like random numbers. Under this assumption ---which is experimentally tested on real-life nets like AlexNet--- it is formally proved that feed forward net is a correct inference method for recovering the hidden layer. The generative model suggests a simple modification for training: use the generative model to produce synthetic data with labels and include it in the training set. Experiments are shown to support this theory of random-like deep nets; and that it helps the training.

==> derivation.tex <==
\section{Derivation of the approximation~\eqref{eqn:log-likelihood}}\label{sec:der} 
We write the log likelihood of $x$ given $h$ under our model (with small gaussian noise added as discussed before), 
$$\log \Pr[x\mid h] \propto\log \sum_{T: |T|=t} \exp(\|x-(r(\alpha Wh))_T\|^2/2\sigma^2)$$
Note that since all the $T$'s of size $t$ are chosen with the same probability, here we have uniform sum of exponentials. In the
spirit of Stochastic Gradient descent, we  do the naive approximation of simply picking a random subset $T$ to approximate the averaging over all $T$'s, and obtain
$$R(W) = \log \Pr[x\mid h] \underset{\sim}{\propto}\|x-(r(\alpha Wh))_T\|^2$$
where $T$ of size $t$ is picked uniformly at random.

We take gradient of $R(W)$ over $W$ and obtain that $\frac{\partial R}{\partial W} \approx \left((x_T-r(Wh)_T)\odot r'(Wh)_T\right)h^T$ where $\odot$ denotes the entry-wise product of two vectors. Therefore taking expectation over the randomness of $T$ again, we obtain that 
$$\nabla_W \log \Pr[x\mid h]  = \Exp_T\left[\frac{\partial R}{\partial W}\right] \approx \left(x  - (r(Wh))\odot r'(Wh)\right)h^T$$
%\Tnote{Yingyu, could you please check whether this is what we used in the code? I am a bit too tired to get the gradient correctly

==> exp_bak.tex <==
% !TEX root = deepnet_main.tex
\vspace{-2mm}
\section{Experiments}
\label{sec:exp}

\begin{figure*}
\centering
\subfigure[CIFAR-10]{
	\includegraphics[width=0.3\textwidth]{figure/cifar10_error} \label{fig:cifar10}
}
\subfigure[CIFAR-100]{
	\includegraphics[width=0.3\textwidth]{figure/cifar100_error} \label{fig:cifar100}
}
%\subfigure[0.2 fraction of CIFAR-10]{
  %\includegraphics[width=0.3\textwidth]{figure/cifar10_error} \label{fig:cifar10f2}
%}
\caption{Error rate v.s. iteration}
\label{fig:exp}
\end{figure*}

%In this section we provide some preliminary experimental results on our model. 
First, we perform a verification of the reversibility property of a random network, since our theorems only are able to prove for three layers. We build a random network of three fully connected layers with random Gaussian followed by ReLU units, with size 128  on the top and increased by a factor of 4 each layer down.  A 0-1 vector with sparsity 4 is generated on the top. Then we follow the generative model to get the bottom layer data, and then follow the inference to recover the top layer vector. All our 1000 trials successfully recovers the support of the top layer vector, which is consistent with our analysis. %We also found that the real life network (e.g alexnet) trained without enforcing 

We then provide some preliminary experimental results on two data sets CIFAR-10 and CIFAR-100~\cite{krizhevsky2009learning}, using the Caffe platform~\cite{jia2014caffe}.  
Four methods are implemented and compared: a baseline, and those combined with our regularization, with dropout, and with both.
The baseline consists of three convolutional layers and three fully connected layers. The three convolutional layers have $96$, $128$, $256$ filters, respectively, %and all use kernel size 5, stride 1 and padding 2. 
followed by ReLU layer and max-pooling layer. %with kernel size 3 and stride 2. 
When dropout is applied, the dropout ratio for the convolutional layers is 0.25, and that for the fully connected layers is 0.5.%, following the suggested values~\cite{Srivastavadropout}. 

For fair comparison, we use the same set of hyperparameters for different methods. The solver script provided by Caffe for CIFAR-10 were adopted, with some modifications: we set the weight decay to be 0.001 to avoid divergence observed in the training, and the learning rate is decreased by 5 every 40,000 iterations. The initial values of our regularization weights and their decay scheme across iterations are determined from a validation set of 5,000 training examples. 
%Following~\cite{Srivastavadropout}, after finding the parameters, the validation set is combined into the training set. 
We preform standard preprocessing by subtracting the mean of the training set. %No other operations such as corner cropping or data argumentation are performed. 

%The CIFAR-10 data set consists of $32 \times 32$ color images drawn from 10 classes, respectively. There are 5,000 training images and 1,000  test images in each class. CIFAR-100 is similar to CIFAR-10 but with 100 classes, and thus is more challenging.  

Figure~\ref{fig:cifar10} shows the error rate on CIFAR-10.  
It can be seen that using our regularization leads to fast increase at the early iterations and also leads to good performance in the late iterations. Figure~\ref{fig:cifar100} shows that  using only our regularization leads to bad performance in this case but combining with dropout outperforms the others, suggesting that it can be useful combined with other regularization. 

==> macro.tex <==
%\renewcommand{\algorithmicrequire}{\bf Input: }
%\renewcommand{\algorithmicensure}{\bf Output: }
\usepackage{amsmath,amsbsy,amsfonts,amssymb,amsthm,dsfont,fullpage,units}
\usepackage{graphicx}
\usepackage{authblk}
\usepackage{algorithm,algorithmic,mathtools}
\usepackage{color,cases}
\usepackage{tikz}
\usetikzlibrary{calc,shapes}
\usepackage{subfigure}
%\usepackage[round]{natbib}
\usepackage{hyperref}
\usepackage{nicefrac}
\newcommand{\sfrac}[2]{#1\nicefrac{}{#2}}

\newtheorem{claim}{Claim}
\newtheorem{corollary}{Corollary}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}[section]
\newtheorem{theorem}{Theorem}[section]
\theoremstyle{definition}
\newtheorem{condition}{Condition}[section]
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
%\theoremstyle{remark}
\newtheorem{remark}{Remark}
%

% % %  define macro for big O star and Omega star

\newcommand{\Os}[1]{= O^*(#1)}
\newcommand{\Oms}[1]{ = \Omega^*(#1)}

 \newcommand{\IGNORE}[1]{}

\newcommand{\citep}{\cite}
\newcommand{\citet}{\cite}
\newcommand{\citealp}{\cite}
\def\nn{\nonumber}

%%%%%from other papers
\newcommand\E{\mathbb{E}}
\newcommand\R{\mathbb{R}}
\newcommand\N{\mathcal{N}}
\def\Pbb{\mathbb{P}}

\renewcommand\t{{\scriptscriptstyle\top}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Astar}{\tilde{A}}
\DeclareMathOperator{\Bstar}{\tilde{B}}
\DeclareMathOperator{\Cstar}{\tilde{C}}
\DeclareMathOperator{\wstar}{\tilde{w}}
\DeclareMathOperator{\astar}{\tilde{a}}
\DeclareMathOperator{\bstar}{\tilde{b}}
\DeclareMathOperator{\cstar}{\tilde{c}}
\newcommand\wh{\widehat}
\newcommand\wt{\widetilde}
%\newcommand\eps{\varepsilon}
%\newcommand\veps{\varepsilon}
\newcommand\h{\hat}

\newcommand\tl{\tilde}
%\newcommand\bar{\overline}
\newcommand\inner[1]{\langle #1 \rangle}
\newcommand\sign{\operatorname{sign}}
\newcommand\poly{\operatorname{poly}}
\newcommand\polylog{\operatorname{polylog}}
\newcommand\supp{\operatorname{supp}}
\newcommand\Proj{\operatorname{Proj}}
\newcommand\Diag{\operatorname{Diag}}
\DeclareMathOperator{\range}{range}
\newcommand{\Exp}{\mathop{\mathbb E}\displaylimits}
\newcommand{\tildO}[1]{\tilde{O}(#1)}
\newcommand{\since}[1]{\textrm{Since #1}}



\newcommand\indicator[1]{\ensuremath{\mathbf{1}_{#1}}}



\def\shownotes{1}  %set 1 to show author notes
\ifnum\shownotes=1
\newcommand{\authnote}[2]{{ $\ll$\textsf{\footnotesize #1 notes: #2}$\gg$}}
\else
\newcommand{\authnote}[2]{}
\fi
\newcommand{\Tnote}[1]{{\authnote{Tengyu}{#1}}}

\newcommand{\hSigma}{\hat{\Sigma}}
\newcommand{\tilM}{\widetilde{M}}
\newcommand{\sca}{\lambda}
\newcommand{\mat}{\textup{mat}}
\newcommand{\uni}{\{\pm1\}^n}
\newcommand{\tilO}{\widetilde{O}}
\newcommand{\tilOmega}{\widetilde{\Omega}}
\newcommand{\polyring}[1]{\mathbb{R}[x]_{#1}}
\newcommand{\s}[1]{(#1)}

==> model_copy.tex <==
% !TEX root = deepnet_main.tex
\vspace*{-0.1in}
\section{Single layer generative model}
\label{sec:model}

For simplicity let's
start with a single layer neural net  $h = r(W^Tx + b),$ where $r$ is the rectifier linear function, $x \in \R^n, h \in \R^m$. When $h$ has fewer nonzero coordinates than $x$, this has to be a many-to one function, and prior work on 
generative models has tried to define a probabilistic inverse of this function.  Sometimes ---e.g., in context of denoising autoencoders--- such inverses are called {\em reconstruction}
if one thinks of all inverses as being similar.
Here we abandon the idea of reconstruction and  focus on defining {\em many} inverses 
$\hat{x}$ of $h$. We define a {\em shadow distribution} $P_{W,\rho}$ for
$x|h$, such that a random sample $\tilde{x}$ from this distribution
satisfies Property (b), i.e., $r(W^T\tilde{x}+ b) \approx h$ where $\approx$ denotes approximate equality of vectors.
To understand the considerations in defining such an inverse, 
one must keep in mind that the ultimate goal is to extend the notion 
 to multi-level nets. Thus a generated \textquotedblleft inverse\textquotedblright~$\tilde{x}$ has to look like the {\em output} of a 1-level net in the layer below. As mentioned, this is  where previous attempts such as DBN or denoising autoencoders run into theoretical difficulties. 
%\iffalse For instance, denoising autoencoders ---using so-called {\em weight-tying}---use the {\em deterministic} inversion  $\hat{x} = Wh$, but then $\hat{x}$ is not sparse  and may have negative coordinates, and thus not look like the output of the RELU layer below. The proposal below 
%fixes this in the obvious way. The more difficult part is ensuring property (b), namely, 
%
%
%\Tnote{Start editing here: }
%\fi 

From now on we use $x$ to denote both the random variable and  a specific sample from the distribution defined by the random variable. Given $h$, sampling $x$ from the distribution $P_{W,\rho}$ consists of first computing $r(\alpha Wh)$ for a scalar $\alpha$ and then randomly zeroing-out each coordinate with probability $1-\rho$. (We refer to this noise model  as \textquotedblleft dropout noise.\textquotedblright) Here  $\rho$ can be reduced to make $x$ as sparse as needed; typically $\rho$ will be small. More formally, we have (with $\odot$ denoting  entry-wise product of two vectors):
\begin{equation}
x = r(\alpha Wh)~\odot n_{\drop}\,,\label{eqn:generative_model}
\end{equation}
where $\alpha = 2/(\rho n)$ is a scaling factor, and $n_{\drop}\in \{0,1\}^n$ is a binary random vector with following probability distribution where $\|n_{\drop}\|_0$ denotes the number of non-zeros of $n_{\drop}$. 
\begin{equation}
\Pr[n_{\drop}] = \rho^{\|n_{\drop}\|_0}.
\end{equation}

Model~\eqref{eqn:generative_model} defines the conditional probability $\Pr[x\vert h]$ (Property (a)). 
The  next informal claim
(made precise in Section~\ref{sec:singlereverse}) shows that Property (b) also holds, 
%ustifies this, 
provided the net (i.e., W) is random-like, and 
%Regarding the distribution of $h$, we only assume 
$h$ is sparse and nonnegative (for precise statement see Theorem~\ref{thm:single}).

\iffalse 
 This alone is sufficient to prove that the single layer net is reversible, that is, Property (b) is satisfied for the joint distribution of $(h,x)$ described above. 
 \fi 
  
 
\begin{theorem}[Informal version of Theorem~\ref{thm:single}]\label{thm:informal}
	If entries of $W$ are drawn from i.i.d Gaussian prior, then for $x$ that is generated from  model~\eqref{eqn:generative_model}, there is a threshold $\theta \in \R$ such that $r(W^T x + \theta \one) \approx h$, where
	$\one$ is the all-$1$'s vector.
\end{theorem}

Section~\ref{sec:multilayer} shows that this  1-layer generative model composes layer-wise while preserving Property (b). The main reason this works is that
the above theorem makes  minimal distributional assumptions about  $h$. 
(In contrast with RBMs where $h$ has a complicated distribution that is difficult to match to the next layer.)

%This is in contrast to RBMs where $h$ has a complicated distribution that is difficult to match to the next layer.


%Our simple change  is to define the inverse using RELU's again: for a suitable $b$, let
%$\hat{x} = r(Wh + b') + \mbox{\em droput noise}$, where the noise consists of randomly zero-ing out a certain fraction of nonzero coordinates. 
%It should be highly unclear why Property (b) is satisfied for the joint distribution of $(h,x)$ described above. 
%such a generative model will be an inverse of the feed-forward neural net, i.e., why it satisfies 
%inverse is well-defined, i.e., satisfies 
%$r(W^Tx+ b') \approx h$. 

%{\em  If entries of $W$ are chosen as iid standard Gaussian, then there is a threshold $\theta \in \Re$ such that $r(W^T \hat{x} + \theta \vec{1}) \approx h$, where
%$\vec{1}$ is the all-$1$'s vector.}

 
% Thus if $W$ is a random matrix, then the feed-forward net finds a vector that is close to the most %likely $h$. 
 
 %This 1-layer generative model composes layer-wise since the Theorem makes essentially no assumption about  $h$ other than sparsity. This is in contrast to RBMs where $h$ has a complicated distribution that is difficult to match to the next layer.
 % the output of the generative model has the same form
 %(each layer a vector of nonnegative numbers) whose sparsity can be tuned to match that of the %utput of the lower layer.
 
 \iffalse 
 Before proceeding further we explain how one should think of the 
 {\em random-like net hypothesis}. Clearly, the edge weights in a real-life net are not random, since
 they are obtained from training. But they could behave enough like random numbers to allow the 
 above theorem to hold. Our experiments suggest that this is the case for real life nets, specifically, the fully connected layers. It is an open question
  why backpropagation finds such random-like nets.
Our experiments also verify another simple prediction of the above informal theorem ---that the 
 threshold vector $b$ of real-life RELU layers is a scalar multiple of $\vec{1}$, the all-$1$ vector. Finally, the dropout noise in the generative model also provides a simple explanation for the efficacy of  dropout in backpropagation training. (We also discuss the application of our theory to convolutional nets later in Section~\ref{}.)
 
  \fi 
  
  
 %It does appear that current training methods find such random-like solutions.

 %\Tnote{Why they run into difficulties? theroetically?}


\subsection{Why random-like nets hypothesis helps theory}
\label{sec:whyrandom}

 
\iffalse 
Then the column vectors of $W^T$ are roughly orthogonal 
(two random unit vectors in $\Re^m$ have inner product of the order of $1/\sqrt{m}$) and so $W W^T$ is roughly like an identity matrix
with $1$'s on the diagonals and low values on the off-diagonal entries. 
Then $W$ is an inverse of sorts for $W^T$, and 
allows recovery of $x$ from $h$ {\em provided $x$ is a sufficiently sparse vector}.
% Thus thinking of inversion as reconstruction seems
But such strong constraints on sparsity etc. don't hold in real-life neural nets.  




\fi 


%To explain the {\em random-like net hypothesis} and why it implies a generative analog of the deep net. Along the way we encounter
%denoising autoencoders and examine why they did not lead to a generative model.



%\Tnote{change to $\tilde{x}$ because somehow $\hat{}$ might be often used as estimator}

%The starting point of the current paper is that one can use $h, W$ to define a very simple probability distributions on This only uses the %random-like nets assumption, and works for much more general values of sparsities of $h, x$. 





%The basic idea is as follows. 
%\Tnote{Start editing here}
%Suppose we have two layer of variables, where $h\in \mathbb{R}^m$ denotes hidden representation of the layer above and $x\in \mathbb{R}^n$ %denotes the observable variables below. 

 Continuing informally, we explain  why the random-like nets hypothesis ensures that the shadow distribution satisfies Property (b).
 % well-defined. \Tnote{I feel it could be not quite clear for what ``well-define" means. We may need to define what does it mean by "well-define" first if we want to use this term. }
  It's helpful to first consider the {\em linear} (and deterministic) generative model sometimes used in autoencoders,  $\hat{x} = Wh$ --- also a subcase of ~\eqref{eqn:generative_model} where $\rho = 1$ and the rectifier linear $r(\cdot)$ is removed. 

Suppose the entries of $W$ are chosen from a distribution with mean $0$ and variance $1$
and are independent of $h$. %(Remember that we are describing a multilayer generative model, so $h$ is generated using the higher layer, which features different edge weights than $W$). 
We now show $\hat{h} = W^T\hat{x}$  is close to $h$ itself up to a proper scaling\footnote{Since RELU function $r$ satisfies  for any nonnegative $\alpha$, $r(\alpha x) = \alpha r(x)$,  readers should from now on basically ignore the positive constant scaling, without loss of generality.}. 

A simple way to show this would be to write $\hat{h} = W^TWh$, and then use the fact that for random Gaussian matrix $W$, the covariance $W^TW$ is approximately the identity matrix. However, to get better insight we work out the calculation more laboriously  so as to  
later allow an intuitive extension to the nonlinear case.
%Readers might want to keep in mind that the arguments below are supposed to demonstrate intuitions and are written in a way that extension to nonlinear case is possible. %Let $\hat{h} = W^T\hat{x}$ be the hidden vector \textit{before} applying the bias shift and RELU and .  
Specifically, rewrite a single coordinate  $\hat{h}_i$  as a linear combination of $\hat{x}_j$'s: 
\begin{equation}
\hat{h}_i = \sum_{j=1}^n W_{ji}\hat{x}_j. \label{eqn:hi}
\end{equation}
By the definition of $\hat{x}_j$, each term on the RHS of~(\ref{eqn:hi}) is equal to 
\begin{equation}
W_{ji}\hat{x}_j = W_{ji}\sum_{\ell=1}^m W_{j\ell}h_{\ell} = \underbrace{W_{ji}^2h_i}_{\textrm{signal:}\mu_j} + \underbrace{W_{ji}\sum_{\ell\neq j}W_{j\ell}h_{\ell}}_{\textrm{noise:}\eta_j}\,.\label{eqn:wjihatxj}
\end{equation}
We split the sum this way to highlight that the first subgroup of terms reinforce each other since 
%of $W_{ji}x_j$ to $\hat{h}_i$.  The term
 $\mu_j = W_{ji}^2 h_i$ is always nonnegative. Thus  $\sum_j \mu_j$ accumulates into a large multiple of $h_i$ and becomes
 the main \textquotedblleft signal\textquotedblright~on the the RHS of~\eqref{eqn:hi}. On the other hand, the noise term $\eta_j$, though it would typically dominate $\mu_j$ in~\eqref{eqn:wjihatxj} in magnitude, has mean zero. Moreover, $\eta_j$ and $\eta_{t}$ for different $j,t$ should be rather independent since they depend on different set of $W_{ij}$'s (though they both depend on $h$). When we sum equation~\eqref{eqn:wjihatxj} over $j$, the term  
 $\sum_j \eta_j$ attenuates due to such cancellation. 
 %and obtain the RHS of~\eqref{eqn:hi} as a sum of $b_j$' and $\sigma_j$'s, %where $b_j$' accumulates and $\sigma_j$
%Given the definition above we can write~\eqref{eqn:hi} as
\begin{equation}
\hat{h}_i = \sum_{j=1}^n \mu_j + \sum_{j=1}^n \eta_j \approx nh_i + R\label{eqn:bias-noise}
\end{equation}
where we used that $\sum_{j}W_{ji}^2  \approx n$, and $R = \sum_j \eta_j$. Since $R$ is a sum of random-ish numbers, due to the averaging effect, it scales as $\sqrt{nm}$. For large $n$ (that is $\gg m$), the signal dominates the noise and we obtain that $\hat{h}_i \approx nh_i$. %Moreover, if we chose $b' \approx -\sqrt{n\log n}$ so that $|b'| > R$ with high probability. Then we obtain that for $i$ with $h_i = 0$, $\tilde{h}_i = r(\hat{h}_i + b) = r(nh_i + R + b)= nh_i$. Similarly we can show that for non-zero $h_i$, $\tilde{h}_i = nh_i \pm O(|b|)$. It follows that $\|\frac{1}{n}\hat{h} - h\|\lesssim \frac{1}{\sqrt{n}}$. 
This argument can be made rigorous to give  the following proposition, whose  proof appears in Section~\ref{app:complet-one-layer}.

\begin{proposition}[Linear generative model]
	Suppose entries $W$ are i.i.d Gaussian. Let $n > m$, and $h \in \{0,1\}^m$, and $\hat{x}$ is generated from the deterministic linear model $x = Wh$, then with high probability,  the recovered hidden variable 
$\hat{h} = W^Tx $ satisfies that $\|\hat{h} - h\|_{\infty} \le \tilde{O}\left(\sqrt{m/n}\right)$
\end{proposition}
%$C = \sum_{j}W_{ji}^2 > 0$ is a constant, and since $\sigma_j$ are mean zero and random-like, we expect the$R = \sum_j \sigma_j$ to be small. 
The biggest problem with this simple linear generative model is that signal  dominates noise in ~\eqref{eqn:bias-noise} only when  $n \gg m$. That is, the feed-forward direction must always reduce dimensionality by a large
factor, say $10$. This is unrealistic, and fixed in the nonlinear model,   with RELU gates playing an important \textquotedblleft denoising\textquotedblright role.

\vspace{-2mm}
\subsection{\bf Formal proof of Single-layer Reversibility}
\label{sec:singlereverse}

%We fix the problems with the above linear inversion with a nonlinear inversion that uses RELUs and
%dropout noise. 
%\iffalse In this section we formally state and prove Theorem~\ref{thm:informal} and its implications under the generative model~\eqref{eqn:generative_model} that describes $\Pr[x\vert h]$. We prove why despite being produced through a nonlinear function $r$ and entry-wise dot product with $n_{\drop}$, the resulting $x$ still enjoys the desired property that $h \approx \relu(W^Tx+b)$ for some properly chosen $b$. 
%\fi 
Now we give a formal version of Theorem~\ref{thm:informal}. We begin by introducing a succinct notation for model~\eqref{eqn:generative_model}, which will be helpful for later sections as well. 
Let $t = \rho n$ be the expected number of non-zeros in the vector $n_{\drop}$, and let $s_t(\cdot)$ be the random function  that drops coordinates with probability $1-\rho$, that is, $s_t(z) =  z \odot n_{\drop}$. Then we rewrite model~\eqref{eqn:generative_model} as 
\begin{equation}
x = s_t(r(\alpha Wh)) \label{eqn:succint}
\end{equation}
%Let $k$ be such that  $h$ is $k$-sparse. 
We make no assumptions on how large  $m$ and $n$ are except to require that $k < t$. Since $t$ is the (expected) number of non-zeros in vector $x$, it is roughly ---up to logarithmic factor--- the amount of \textquotedblleft information\textquotedblright in $x$. Therefore the assumption that $k < t$ is in accord with the usual \textquotedblleft bottleneck\textquotedblright\  intuition, which says that the representation at higher levels has fewer bits of information. 




%We will allow $m > n$ so long as $h$ is $k$-sparse with $k < n$. (This is in accord with the usual \textquotedblleft bottleneck\textquotedblright\  intuition, which says that the representation at higher levels has fewer
%bits of information.) 
%With this assumption, the dimension of the hidden variable could be larger than that of the observation, though the intrinsic dimension (or %information) reduces by going up the layers. 
%The model first applies rectifier linear function over $\alpha\hat{x} = \alpha Wh$ and obtains $\tilde{x} = r(\alpha\hat{x}) = \relu(\alpha Wh)$, where $\alpha = 2/t$ is a scaling constant. 
%Then it applies a random sampling function $s_t(\cdot)$ on $\tilde{x}$ and obtains 
%\begin{equation}
%x = s_t(\tilde{x})  = s_t(r(\alpha Wh)) \label{eqn:generative-one-layer}
%\end{equation}
%Here a random sampling function $s_t(\cdot)$ simply picks randomly a subset of indices $T$ with size $t$ and drops (zero-outs) the values outside support $T$. 



%\footnote{We note that in the feedforward neural network, the choice of $b$ is largely determined by the relative shifts and magnitude of $W$, and the exact choice is not of importance. Therefore it doesn't make much sense to ask for a generative model for any pair $(W,b)$. Or in that case, we allow us the choice of using potentially a different $b$ to calculate hidden representation feedforwardly.%Therefore we think of a feedforward neural network is unique determined by $W$ with some associate $b$. }
 %$b$. %\Tnote{Added the footnote here}
 
% \Snote{Say that $b$ is scalar multiple of $\vec{1}$?}
 
\iffalse 

In this section,we prove that the feedforward calculation on the generated $x$ recovers the hidden variable $h$ approximately.
\fi  
The random-like net hypothesis here  means that the entries of $W$ independently satisfy
$W_{ij}\sim \mathcal{N}(0,1)$.
%We formalize the calculation above in the following theorem. Mathematically to make the argument above formally, we need to prove that sum of $\sigma_j$'s behaves like a gaussian for most of $h$. We assume that the entries of $W$ is drawn from a random gausain prior, that is, 
\begin{equation}
W_{ij}\sim \mathcal{N}(0,1) \label{eqn:prior}
\end{equation}
%where $W_{ij}$ are independent with each other. 
%Then we have the following theorem
%Then we assume that $h$ has a distribution $\mathcal{D}_h$ over $k$-sparse vectors, 
Also we assume the hidden variable $h$ comes from any distribution $D_h$ that is supported on nonnegative $k$-sparse vectors for some $k$,  where none of the nonzero coordinates are very dominant.
(Allowing a few large coordinates wouldn't kill the theory but the notation and math gets hairier.) 
Technically, when $h\sim D_h$, 
\begin{eqnarray}
h \in \mathbb{R}_{\ge 0}^n, \quad |h|_0 \le k \,\textrm{ and }\, |h|_{\infty} \le \beta\cdot \|h\|\quad \textrm{almost surely} \label{eqn:hdistribution}
\end{eqnarray}
where $\beta = O(\sqrt{(\log k)/k}\ )$. The last assumption essentially says that all the coordinates of $h$ shouldn't be too much larger than the average (which is $1/\sqrt{k} \cdot \|h\|$). 
As mentioned earlier the weak assumption on $D_h$ is the key to  layerwise composability.
\begin{theorem}[Reversibility]\label{thm:single}
	Suppose $t = \rho n$ and $k$ satisfy that $k < t < k^2$. 
	For $(1-n^{-5})$ measure of $W$'s, there exists offset vector $b$, such that the following holds:
	%Then there exists offset vector $b$, such that for a typical\footnote{By this we mean that with high probability over the randomness of the prior measure of $W$, the statement of the theorem is true} $W$ from the prior~\eqref{eqn:prior}, 
	when $h\sim D_h$ and $\Pr[x\vert h]$  is specified by model~\eqref{eqn:generative_model}, then with high probability over the choice of $(h,x)$, 
%	\begin{equation}
%	\Pr\left[\|r(W^Tx+b) - h\|^2 \le \tilde{O}(k/(\rho n))\cdot \|h\|\right] \ge 1 - 1/\poly(n)
%	\end{equation}
	\begin{equation}
\|r(W^Tx+b) - h\|^2 \le \widetilde{O}(k/t)\cdot \|h\|^2,.\label{eqn:reversible}
%	
	\end{equation}
	%\|h-\tilde{h}\|^2 \le \widetilde{O}(k/t)\cdot \|h\|\label{eqn:reversible}
	%	
%	for $h\sim D_h$ that satisfies~\eqref{eqn:hdistribution}, and $x = s_t(r(\alpha Wh))$ drawn from generative model~\eqref{eqn:generative_model}, and $k < t < k^2$, %we have that for most of the $k$-sparse $h$, 
%	we have that with high probability over the randomness of $h$ and $x$, 
%	the vector $\tilde{h} = r(W^Tx + b)$ satisfies
%	$
%	\|h-\tilde{h}\|^2 \le \widetilde{O}(k/t)\cdot \|h\|\label{eqn:reversible}
%	$. 
	%For any fixed $h$ with $|h|_0 = k\ll t$ and $\|h\|_{\infty}\ll \|h\|_2$, for $\alpha = \frac{2}{t}$ and some $b$ with $\tilOmega(\frac{\|h\|}{\sqrt{t}})\le b < \frac{1}{2}$, with high probability over the randomness of $W$, $\tilde{h}$ satisfies that $$\|h-\tilde{h}\|^2\le \tilO\left(\frac{k}{t}\right)\|h\|^2$$ %for $\hat{h} = \alpha W^Tx$  with the scaling constant $\alpha = \frac{2}{s}$, we have that $|\hat{h}-h|_{\infty} \le \tilO\left(\frac{\|h\|}{\sqrt{s}}
	%\right)+ \tilO\left(\frac{1}{\|h\|^3}\right)$
\end{theorem} 
%\begin{theorem}[Reversibility]\label{thm:single}
%	There exists offset vector $b$, such that for a typical\footnote{By this we mean that with high probability over the randomness of the prior measure of $W$, the statement of the theorem is true} $W$ from the prior~\eqref{eqn:prior}, for $h\sim D_h$ that satisfies~\eqref{eqn:hdistribution}, and $x = s_t(r(\alpha Wh))$ drawn from generative model~\eqref{eqn:generative_model}, and $k < t < k^2$, %we have that for most of the $k$-sparse $h$, 
%	we have that with high probability over the randomness of $h$ and $x$, 
%	the vector $\tilde{h} = r(W^Tx + b)$ satisfies
%	$
%		\|h-\tilde{h}\|^2 \le \widetilde{O}(k/t)\cdot \|h\|\label{eqn:reversible}
%	$. 
%	%For any fixed $h$ with $|h|_0 = k\ll t$ and $\|h\|_{\infty}\ll \|h\|_2$, for $\alpha = \frac{2}{t}$ and some $b$ with $\tilOmega(\frac{\|h\|}{\sqrt{t}})\le b < \frac{1}{2}$, with high probability over the randomness of $W$, $\tilde{h}$ satisfies that $$\|h-\tilde{h}\|^2\le \tilO\left(\frac{k}{t}\right)\|h\|^2$$ %for $\hat{h} = \alpha W^Tx$  with the scaling constant $\alpha = \frac{2}{s}$, we have that $|\hat{h}-h|_{\infty} \le \tilO\left(\frac{\|h\|}{\sqrt{s}}
%	%\right)+ \tilO\left(\frac{1}{\|h\|^3}\right)$
%\end{theorem} 
%\Snote{Why not say whp over choice of W as well? }


%\Tnote{Sanjeev, could you see if the phrasing of the theorem okay? It is not very rigourous since I am using  ``for a typical $W$ from the prior" }
The next theorem says that the generative model predicts that the trained net should be stable to dropout. 

\begin{theorem}[Dropout Robustness]\label{thm:dropout}
	Under the condition of Theorem~\ref{thm:single}, suppose we further drop 1/2 fraction of values of $x$ randomly and obtain $x^{\textrm{drop}}$, then there exists some offset vector $b'$, such that with high probability over the randomness of $(h,x^{\drop})$, %$x$ and $x^{\textrm{drop}}$, 
	%for $\tilde{h}^{\textrm{drop}} = r(2W^Tx^{\textrm{drop}} + b')$
%	we have 
%		$\|h-\tilde{h}^{\textrm{drop}} \|^2 \le \tilO(k/t)\cdot \|h\|$.
we have 
\begin{equation}
\|r(2W^Tx^{\textrm{drop}} + b')- h\|^2 \le \tilO(k/t)\cdot \|h\|^2.
\end{equation}

\end{theorem}
%\Tnote{ToDo: needs to check whether we say $t = \rho n$ is the expected sparsity of $x$ somewhere. }

To parse the theorems, we note that the error is on the order of the sparsity ratio $k/t$ (up to logarithmic factors), which is necessary since information theoretically the generative direction must increase the amount of information so that good inference is possible. In other words, our theorem shows that under our generative model, feedforward calculation (with or without dropout) can estimate the hidden variable up to a small error when $k \ll t$. Note that this is 
%this doesn't necessarily mean that we can solve
different from usual notions in generative models such as MAP or MLE inference. We get direct guarantees on the estimation error which neither MAP or MLE can guarantee\footnote{Under the situation where MLE (or MAP) is close to the true $h$, our neural-net inference algorithm is also guaranteed to be the close to both MLE (or MAP) and the true $h$.}. %solves the inference problem (even with dropout) approximately when $k\ll t$.  %the error between feedforward representation $\tilde{h}$ (or the dropout version $\tilde{h}^{\drop})$) and the true hidden variable is 

%\Snote{Maybe address the NIPS reviewer question about what is the meaning of solving the inference problem. MAP etc.}

Furthermore, in Theorem~\ref{thm:dropout}, we need to choose a scaling of factor 2 to compensate the fact that  half of the signal $x$ was dropped. Moreover, we remark that an interesting feature of our theorems is that we show an almost uniform offset vector $b$ (that is, $b$ has almost the same entries across coordinate) is enough. This matches the observation  that in the trained Alex net~\cite{ImageNet}, for most of the layers the offset vectors are almost uniform\footnote{Concretely, for the simple network we trained using implementation of~\cite{jia2014caffe}, for 5 out of 7 hidden layers, the offset vector is almost uniform with mean to standard deviation ratio larger than 5. For layer 1, the ratio is about 1.5 and for layer 3 the offset vector is almost 0.}. In our experiments (Section~\ref{sec:exp}), we also found restricting the bias terms in RELU gates to all be some constant makes almost no change to the performance. 
%\Tnote{Need to decide whether to amphasize this}
%\Tnote{Edited here. }


%\Tnote{A tentative sketch}
%Now we provide the proof for Theorem~\ref{thm:single}. 
We devote the rest of the sections to sketching a proof of Theorems~\ref{thm:single} and~\ref{thm:dropout}. 
The main intermediate step of the proof is the following lemma, which will be proved at the end of the section: 

\begin{lemma}\label{lem:beforerelu}
	Under the same setting as Theorem~\ref{thm:single}, with high probability over the choice of $h$ and $x$, we have that for $\delta = \widetilde{O}(1/\sqrt{t})$, 
	\begin{equation}
	\|W^Tx - h \|_{\infty} \le \delta \|h\|\label{eqn:infinitenorm}\,.
	\end{equation}
\end{lemma}

Observe that since $h$ is $k$-sparse, the average absolute value of the non-zero coordinates of $h$ is $\tau = \|h\|/\sqrt{k}$. Therefore the entry-wise error $\delta\|h\|$ on RHS of~\eqref{eqn:infinitenorm} satisfies $\delta\|h\|= \epsilon \tau$ with $\epsilon = \widetilde{O}(\sqrt{k/t})$. %That is, the hidden state before offset and RELU, $W^Tx$,  is close to $h$ with entry-wise error  $\epsilon \tau$. T
This means that $W^Th$ (the hidden state before offset and RELU) estimates the non-zeros of $h$ with entry-wise relative error $\epsilon$ (in average), though the relative errors on the zero entries of $h$ are huge. Therefore, even though we get a good estimate of $h$ in $\ell_{\infty}$ norm, the $\ell_2$ norm of the difference $W^Tx -h$ could be as large as $\epsilon \tau \sqrt{n}  = \widetilde{O}(\sqrt{m/t})\|h\|$ which could be larger than $\|h\|$. % ($\ell_2$ norm error is needed for )

It turns out that the offset vector $b$ and RELU have the denoising effects that reduce errors on the non-support of $h$ down to 0 and therefore drive the $\ell_2$ error down significantly. The following proof of Theorem~\ref{thm:single} (using Lemma~\ref{lem:beforerelu}) formalizes this intuition. 
\begin{proof}[Proof of Theorem~\ref{thm:single}]
		Let $\check{h} = W^Tx$. By Lemma~\ref{lem:beforerelu}, we have that $|\check{h}_i - h_i| \le \delta \|h\|$ for any $i$. Let $b = -\delta\|h\|$. For any $i$ with $h_i = 0$, $\check{h}_i + b \le h_i + \delta \|h\| + b \le 0$, and therefore $r(\check{h}_i + b ) = 0 = h_i$. On the other hand, for any $i$ with $h_i \neq 0$, we have $|\check{h}_i + b  - h_i| \le |b| + |\check{h}_i - h_i|\le 2\delta \|h\|$. It follows that  $|r(\check{h}_i + b)  - r(h_i)| \le 2\delta \|h\|$. Since $h_i$ is nonnegative, we have that $|r(\check{h}_i + b)  - h_i| \le 2\delta \|h\|$. Therefore the $\ell_2$ distance between $r(W^Tx+b) = r(\check{h}+b)$ and $h$ can be bounded by 
		%To finish, we show that taking another rectifier linear on $\alpha\check{h}$ will further reduce the noise. Suppose $h$ has support $K$ of size $k$. We choose $\tilde{b} = -\epsilon\mathbf{1}$, and let $\tilde{h}  =\relu(\check{h} +  \tilde{b}) = \relu(W^Th + \tilde{b})$, then we obtain that for $i\not \in K$,  $\tilde{h}_i  = r(\check{h}_i ) = r(h_i\pm \epsilon + b) = 0$. Therefore, for those $i\not\in K$, there is no loss $\tilde{h}_i = h_i  = 0$. Moreover, this addition nonlinear operation doesn't incur more loss on $K$ either -- for any $i$, it is guaranteed that $|\tilde{h}_i - h_i| \le |\tilde{h_i}-\check{h}_i|+|\check{h}_i- h_i|\le 2\epsilon$. Therefore the total error between $\tilde{h}$ and $h$ in euclidean distance can be bounded by %Therefore using rectifier linear with a small shift $b \approx \epsilon$, the resulting $\tilde{h}$ is exactly equal to 0 when $h_i = 0$, and for $h_i \neq 0$, it only introduce at most another small error $\epsilon$. Therefore then we have that 
		%\begin{equation}
		$\|r(\check{h}+b) - h\|^2 = \sum_{i : h_i \neq 0} |r(\check{h}_i + b)  - h_i|^2 \le 4k \delta^2 \|h\|^2$. Plugging in $\delta = \widetilde{O}(1/\sqrt{t})$ we obtain the desired result. 
\end{proof}
Theorem~\ref{thm:dropout} is a direct consequence of Theorem~\ref{thm:single}, essentially due to the dropout nature of our generative model (we sample in the generative model which connects to dropout naturally). See Section~\ref{app:complet-one-layer} for its proof. 
We conclude with a proof sketch  of Lemma~\ref{lem:beforerelu}. The complete proof can be found in Section~\ref{app:complet-one-layer}. 
\begin{proof}[Proof Sketch of Lemma~\ref{lem:beforerelu}]

	Here due to page limit, we give a high-level proof sketch that demonstrates the key intuition behind the proof, by skipping most of the tedious parts. See section~\ref{app:complet-one-layer} for full details. 
	
	By a standard Markov argument, we claim that it suffices to show that w.h.p over the choice of ($(W,h,x)$ the network is reversible, that is, 
	$
	\Pr_{x,h,W}\left[\textrm{equation~\eqref{eqn:reversible} holds}\right] \ge 1 - n^{10}\,.
	$
	%Indeed, suppose~\eqref{eqn:joint-prob} is true, then using a standard Markov argument, we obtain  
	%$$\Pr_{W}\left[\Pr_{x,h}\left[\textrm{equation~\eqref{eqn:reversible} holds} \mid W\right] > 1-n^{-5} \right]\ge 1 - n^{5},$$ as desired. 
	%Equation~(\ref{eqn:joint-prob}) is proven rigorously in Theorem~\ref{thm:single-technical} in supplementary materials, though here we give a proof sketch that demonstrates the idea. 
	Towards establishing this, we note that equation~\eqref{eqn:reversible} %(and consequently statement~\eqref{eqn:joint-prob}) 
	holds for any positive scaling of $h,x$ simultaneously, since RELU has the property that $r(\beta z) = \beta \cdot r(z)$ for any $\beta \ge 0$ and any $z\in \mathbb{R}$.  Therefore WLOG we can choose a proper scaling of $h$ that is convenient to us. We assume $\|h\|_2^2 = k$. By assumption~\eqref{eqn:hdistribution}, we have that $|h|_{\infty}\le \widetilde{O}(\sqrt{\log k})$. 
	
	Define $\check{h} = \alpha W^Tx$. Similarly to~\eqref{eqn:hi}, we fix $i$ and expand the expression for $\check{h}_i$ by definition, 
	\begin{equation}
	\check{h}_i  = \alpha\sum_{j=1}^n W_{ji}x_j 
	\end{equation}	
	Suppose $n_{\drop}$ has support $T$.  Then we can write $W_{ji}x_j$ as 
	\begin{align}
	W_{ji}x_j  &=  W_{ji}\relu(\sum_{\ell=1}^m W_{j\ell} h_{\ell}) \cdot n_{\drop,j}=  W_{ji}\relu(W_{ji} h_i + \eta_j)\cdot \mathbf{1}_{j\in T} \,,\label{eqn:eqn29-main}
	\end{align}
	where $\eta_j \triangleq \sum_{\ell\neq j}W_{j\ell}h_{\ell}$. Though $\relu(\cdot)$ is nonlinear, it is piece-wise linear and more importantly still Lipschitz. Therefore intuitively, RHS of~\eqref{eqn:eqn29-main} can be ``linearized" by approximating 
	$	\relu(W_{ji}h_i + \eta_j) $ by $\mathbf{1}_{\eta_j > 0}\cdot \left(W_{ji}h_i + \relu(\eta_j)\right)$. 
	%	\begin{equation}
	%	\relu(W_{ji}h_i + \eta_j) \approx  \mathbf{1}_{\eta_j > 0}\cdot W_{ji}h_i + \relu(\eta_j) \label{eqn:approx}
	%	\end{equation}
	Note that this approximation is not accurate only when $|\eta_j|\le |W_{ji}h_i|$, which happens with relatively small probability, since $\eta_j$ typically dominates $W_{ji}h_{i}$ in magnitude. 
	
	%Under this approximation, we found that 
	Then $W_{ji}x_j$ can be written approximately as $\mathbf{1}_{\eta_j > 0}\cdot \left(W_{ji}^2h_i + W_{ji}\relu(\eta_j)\right)$, where the first term corresponds to the bias and the second one corresponds to the noise (variance), similarly to the argument in the linear generative model case in Section~\ref{sec:whyrandom}. 
	
	Using the intuition above, one can formally prove (as in the full proof in Section~\ref{app:complet-one-layer}) that $\Exp[W_{ji}x_j] =\frac{1}{2} h_i \pm \widetilde{O}(1/k^{3/2})$ and $\Var[W_{ji}x_j] = O(\sqrt{k/t})$. By a concentration inequality\footnote{Note that to apply concentration inequality, independence between random variables is needed. Therefore technically, we need to condition on $h$ and $T$ before applying concentration inequality, as is done in the full proof of this lemma in Section~\ref{app:complet-one-layer}. } for the sum  $\check{h}_i = \alpha\sum_{j=1}^n W_{ji}x_j $, one can show that 		
		%(note that  while $W_{ji}h_i$ is only one term while $\eta_j = \sum_{\ell\ne i}W_{j\ell}h_{\ell}$ is a sum, therefore the latter typically dominates the former).
%		Using the intuition above, we can formally calculate the expectation of $W_{ji}x_j$ via a slightly tighter and more sophisticated argument: Conditioned on $h$, we have $W_{ji}\sim\mathcal{N}(0,1)$ and  $\eta_j = \sum_{\ell\neq j}W_{j\ell}h_{\ell} \sim \mathcal{N}(0,\sigma^2)$ with $\sigma^2 = \|h\|^2 - h_j^2 = k - h_j^2 \ge \Omega(k)$. Therefore we have $\log \sigma = \frac{1}{2}\log (\Omega(k)) \ge h_j$ and then by Lemma~\ref{lem:exp} ($W_{ji}$ here corresponds to $w$ in Lemma~\ref{lem:exp}, $\eta_j$ to $\xi$ and $h_j$ to $h$), we have 
%		$
%		\Exp[W_{ji}x_j \mid h] = \Exp[W_{ji}r(W_{ji}h_j + \eta_j) \mid h] = \frac{1}{2} h_j \pm \widetilde{O}(1/k^{3/2})\nonumber
%		$. 
%		It follows that 
%		\begin{equation}
%		\Exp[\check{h}_i\vert h,T] = \sum_{j\in T} \Exp[W_{ji}r(W_{ji}h_j + \eta_j) \mid h] = \frac{\alpha |T|}{2}  h_i \pm \widetilde{O}(\alpha n/k^{3/2})\nonumber
%		\end{equation}
%		
	%	Taking expectation over the choice of $T$ we obtain that $\Exp[\check{h}_i\vert h] = \frac{\alpha t}{2}  h_i \pm \widetilde{O}(\alpha n/k^{3/2}) = h_i \pm \widetilde{O}(1/(tk^{3/2})) $. (Recall that $t = \rho n$ and $\alpha = 2/(\rho n)$. Similarly, the variance of $\check{h}_i\vert h$ can be bounded by 
		%$\Var[\check{h}_i \vert h] = O(k/t)$ (see Claim~\ref{lem:app:var}). Therefore we expect that $\check{h}_i$ concentrate around its mean with fluctuation $\pm O(\sqrt{k/t})$. Indeed, by 
		%	
		%	Equation~(\ref{eqn:approx}) implies that $W_{ji}x_j$ can be written approximately as 
		%	\begin{align}
		%	W_{ji}x_j % &= W_{ji}\cdot \relu(\sum_{\ell}\cdot W_{j\ell}x_{\ell}) \cdot \mathbf{1}_{j\in T} \nonumber\\
		%	& \approx \underbrace{W_{ji}^2h_i \cdot \mathbf{1}_{\eta_j > 0}\cdot \mathbf{1}_{j\in T}}_{\textrm{signal: } \mu_j'}  +\underbrace{W_{ji}r(\eta_j)\cdot \mathbf{1}_{j\in T} }_{\textrm{noise: } \eta_j'} 
		%	\end{align}
		%Though here we have a more complicated formula than~\eqref{eqn:wjihatxj}, actually the same intuition applies: when taking sum of $W_{ji}x_j$ over $j$, $u_j'$ contributes to the signal term, while the sum of $W_{ji}r(\eta_j')$ attenuates due to cancellation (note that it is still mean zero due to the fact $W_{ji}$ is mean zero and independent with $r(\eta_j')$. %has mean zero and contributes the variance, and we obtain that 
	%	by concentration inequality, we can prove (see Lemma~\ref{lem:concentration} in Section~\ref{app:complet-one-layer}) that actually $\check{h}_i\mid h$ is sub-Gaussian, and therefore  conditioned on $h$, 
	with high probability ($1-n^{-10}$) we have $|\check{h}_i -  h_i| \le \widetilde{O}(\sqrt{k/t})$.  %, where the first term account for the variance and the second is due to the bias (difference between $\Exp[\check{h}_i]$ and $h_i$). 
		%$$\Pr\left[|\check{h}_i -  h_i| \ge \widetilde{\Omega}((\sqrt{k/t}+ 1/(tk^{3/2}))\mid h\right] \le n^{-10}\,.$$		
		%Noting that $k < t < k^2$ and therefore $1/(tk^{3/2})$ is dominated by $\sqrt{k/t}$, take expectation over $h$, we obtain that $\Pr\left[|\check{h}_i -  h_i| \ge \widetilde{\Omega}(\sqrt{k/t})\right] \le n^{-10}$. 
		Taking union bound over all $i\in [n]$, we obtain that with high probability, $\|\check{h} - h\|_{\infty} \le \widetilde{O}(\sqrt{k/t})$.  Recall that $\|h\|$ was assumed to be equal to $k$ (WLOG). Hence we obtain that $\|\check{h} - h\|_{\infty} \le \widetilde{O}(\sqrt{1/t})\|h\|$ as desired. 
\end{proof}
%Therefore $\tilde{x}$ is still nonnegative so that potentially we can compose another layer below. 


%We see that $W_{ji}\hat{x}_j$ contains 




%Our generative model works as follows:  Given $h$, suppose we generate $\tilde{x} = W^Th$ 
%we first compute $\hat{x} = \relu(W^Tx+b)$

%Suppose for some $\tilde{x}$ it is true that $r(W\tilde{x} + b) = h$. We fix some index $i$ such that $h_i > 0$. 
\iffalse 
But there is a an inverse of sorts exists if $W$ is random-like. To see this first imagine the mapping is linear, $h = Wx$, and


Suppose  and the columns are unit vectors. Then the columns have small pairwise inner products of around 
$1/\sqrt{m}$ (since random vectors tend to have low inner products) and thus $W^T W$ is an $n \times n$ matrix that has $1$'s on the diagonal and low values around $1/\sqrt{m}$ on the off-diagonals. Thus if $x$ has at most $??$ nonzero entries, 
\fi 
 

==> proofsketch.tex <==
Here due to page limit, we give a high-level proof sketch that demonstrates the key intuition behind the proof, by skipping most of the tedious parts. See section~\ref{app:complet-one-layer} for full details. 

By a standard Markov argument, we claim that it suffices to show that w.h.p over the choice of ($(W,h,x)$ the network is reversible (that is, ~\eqref{eqn:reversible} holds), 
\begin{equation}
\Pr_{x,h,W}\left[\textrm{equation~\eqref{eqn:reversible} holds}\right] \ge 1 - n^{10}\,.\label{eqn:joint-prob}
\end{equation}
%Indeed, suppose~\eqref{eqn:joint-prob} is true, then using a standard Markov argument, we obtain  
%$$\Pr_{W}\left[\Pr_{x,h}\left[\textrm{equation~\eqref{eqn:reversible} holds} \mid W\right] > 1-n^{-5} \right]\ge 1 - n^{5},$$ as desired. 
%Equation~(\ref{eqn:joint-prob}) is proven rigorously in Theorem~\ref{thm:single-technical} in supplementary materials, though here we give a proof sketch that demonstrates the idea. 
Towards establishing~\eqref{eqn:joint-prob}, we note that equation~\eqref{eqn:reversible} (and consequently statement~\eqref{eqn:joint-prob}) holds for any positive scaling of $h,x$ simultaneously, since RELU has the property that $r(\beta z) = \beta \cdot r(z)$ for any $\beta \ge 0$ and any $z\in \mathbb{R}$.  Therefore WLOG we can choose a proper scaling of $h$ that is convenient to us. We assume $\|h\|_2^2 = k$. By assumption~\eqref{eqn:hdistribution}, we have that $|h|_{\infty}\le \widetilde{O}(\sqrt{\log k})$. 

Define $\check{h} = \alpha W^Tx$. Similarly to~\eqref{eqn:hi}, we fix $i$ and expand the expression for $\check{h}_i$ by definition and obtain 
\begin{equation}
\check{h}_i  = \alpha\sum_{j=1}^n W_{ji}x_j 
\end{equation}	
%Suppose the random sampling function $s_t(\cdot)$ drops all the values outside support $T$, we can write $x_j$ as 
Suppose $n_{\drop}$ has support $T$.  Then we can write $W_{ji}x_j$ as 
\begin{align}
W_{ji}x_j  &=  W_{ji}\relu(\sum_{\ell=1}^m W_{j\ell} h_{\ell}) \cdot n_{\drop,j}=  W_{ji}\relu(W_{ji} h_i + \eta_j)\cdot \mathbf{1}_{j\in T} \,,\label{eqn:eqn29}
\end{align}
where $\eta_j \triangleq \sum_{\ell\neq j}W_{j\ell}h_{\ell}$. Though $\relu(\cdot)$ is nonlinear, it is piece-wise linear and more importantly still Lipschitz. Therefore intuitively, RHS of~\eqref{eqn:eqn29} can be ``linearized" by approximating 
$	\relu(W_{ji}h_i + \eta_j) $ by $\mathbf{1}_{\eta_j > 0}\cdot \left(W_{ji}h_i + \relu(\eta_j)\right)$. 
%	\begin{equation}
%	\relu(W_{ji}h_i + \eta_j) \approx  \mathbf{1}_{\eta_j > 0}\cdot W_{ji}h_i + \relu(\eta_j) \label{eqn:approx}
%	\end{equation}
Note that this approximation is not accurate only when $|\eta_j|\le |W_{ji}h_i|$, which happens with relatively small probability, since $\eta_j$ typically dominates $W_{ji}h_{i}$ in magnitude. 

Under this approximation, we found that $W_{ji}x_j$ can be written approximately as $\mathbf{1}_{\eta_j > 0}\cdot \left(W_{ji}^2h_i + W_{ji}\relu(\eta_j)\right)$, where the first term corresponds to the bias and the second one corresponds to the noise (variance), similarly to the argument in the linear generative model case in Section~\ref{sec:whyrandom}. 

Using the intuition above, one can formally prove (as in the full proof in Section)

%(note that  while $W_{ji}h_i$ is only one term while $\eta_j = \sum_{\ell\ne i}W_{j\ell}h_{\ell}$ is a sum, therefore the latter typically dominates the former).

Using the intuition above, we can formally calculate the expectation of $W_{ji}x_j$ via a slightly tighter and more sophisticated argument: Conditioned on $h$, we have $W_{ji}\sim\mathcal{N}(0,1)$ and  $\eta_j = \sum_{\ell\neq j}W_{j\ell}h_{\ell} \sim \mathcal{N}(0,\sigma^2)$ with $\sigma^2 = \|h\|^2 - h_j^2 = k - h_j^2 \ge \Omega(k)$. Therefore we have $\log \sigma = \frac{1}{2}\log (\Omega(k)) \ge h_j$ and then by Lemma~\ref{lem:exp} ($W_{ji}$ here corresponds to $w$ in Lemma~\ref{lem:exp}, $\eta_j$ to $\xi$ and $h_j$ to $h$), we have 
$
\Exp[W_{ji}x_j \mid h] = \Exp[W_{ji}r(W_{ji}h_j + \eta_j) \mid h] = \frac{1}{2} h_j \pm \widetilde{O}(1/k^{3/2})\nonumber
$. 

It follows that 
\begin{equation}
\Exp[\check{h}_i\vert h,T] = \sum_{j\in T} \Exp[W_{ji}r(W_{ji}h_j + \eta_j) \mid h] = \frac{\alpha |T|}{2}  h_i \pm \widetilde{O}(\alpha n/k^{3/2})\nonumber
\end{equation}

Taking expectation over the choice of $T$ we obtain that $\Exp[\check{h}_i\vert h] = \frac{\alpha t}{2}  h_i \pm \widetilde{O}(\alpha n/k^{3/2}) = h_i \pm \widetilde{O}(1/(tk^{3/2})) $. (Recall that $t = \rho n$ and $\alpha = 2/(\rho n)$. Similarly, the variance of $\check{h}_i\vert h$ can be bounded by 
$\Var[\check{h}_i \vert h] = O(k/t)$ (see Claim~\ref{lem:app:var}). Therefore we expect that $\check{h}_i$ concentrate around its mean with fluctuation $\pm O(\sqrt{k/t})$. Indeed, by 
%	
%	Equation~(\ref{eqn:approx}) implies that $W_{ji}x_j$ can be written approximately as 
%	\begin{align}
%	W_{ji}x_j % &= W_{ji}\cdot \relu(\sum_{\ell}\cdot W_{j\ell}x_{\ell}) \cdot \mathbf{1}_{j\in T} \nonumber\\
%	& \approx \underbrace{W_{ji}^2h_i \cdot \mathbf{1}_{\eta_j > 0}\cdot \mathbf{1}_{j\in T}}_{\textrm{signal: } \mu_j'}  +\underbrace{W_{ji}r(\eta_j)\cdot \mathbf{1}_{j\in T} }_{\textrm{noise: } \eta_j'} 
%	\end{align}
%Though here we have a more complicated formula than~\eqref{eqn:wjihatxj}, actually the same intuition applies: when taking sum of $W_{ji}x_j$ over $j$, $u_j'$ contributes to the signal term, while the sum of $W_{ji}r(\eta_j')$ attenuates due to cancellation (note that it is still mean zero due to the fact $W_{ji}$ is mean zero and independent with $r(\eta_j')$. %has mean zero and contributes the variance, and we obtain that 
by concentration inequality, we can prove (see Lemma~\ref{lem:concentration} in Section~\ref{app:complet-one-layer}) that actually $\check{h}_i\mid h$ is sub-Gaussian, and therefore  conditioned on $h$, with high probability ($1-n^{-10}$) we have $|\check{h}_i -  h_i| \le \widetilde{O}((\sqrt{k/t}+ 1/(tk^{3/2}))$, where the first term account for the variance and the second is due to the bias (difference between $\Exp[\check{h}_i]$ and $h_i$). 
%$$\Pr\left[|\check{h}_i -  h_i| \ge \widetilde{\Omega}((\sqrt{k/t}+ 1/(tk^{3/2}))\mid h\right] \le n^{-10}\,.$$

Noting that $k < t < k^2$ and therefore $1/(tk^{3/2})$ is dominated by $\sqrt{k/t}$, take expectation over $h$, we obtain that $\Pr\left[|\check{h}_i -  h_i| \ge \widetilde{\Omega}(\sqrt{k/t})\right] \le n^{-10}$. Taking union bound over all $i\in [n]$, we obtain that with high probability, $\|\check{h} - h\|_{\infty} \le \widetilde{O}(\sqrt{k/t})$.  Recall that $\|h\|$ was assumed to be equal $k$ without loss of generality. Hence we obtain that $\|\check{h} - h\|_{\infty} \le \widetilde{O}(\sqrt{1/t})\|h\|$ as desired. 

==> reg.tex <==
% !TEX root = deepnet_main.tex
\vspace{-2mm}
\section{Implications for Regularization}
\label{sec:reg}


\cite{Srivastavadropout} provide two appealing intuitions for using dropout training: (a) it penalizes {\em complex co-adaption} of features within the deep net, so that no feature relies upon a complex firing of other features to do its work.
(b) it is an efficient way of model averaging, which effectively averages over exponentially many good networks. 

Our theory is consistent with these views. The random-like net assumption can be seen as an attempt to formalize (a), since random-like features
by definition have no significant correlations. 
The generative model following from our theory can be seen as some theoretical justification for (b).
The generative model randomly zeroes out entries, which is similar to being an average of exponentially many subnetworks.
It provably is robust to dropout.
%any dropout of the network wont' significantly change the performance of the network on $x$. 

\iffalse net assumption. The mystery about the model averaging view is:  s? Our generative model shows that this can be made precise 
it is entirely possible and actually very often to occur -- as long as the net is random like, for most the observables $x$ generated from our generative model,\fi
 

\iffalse Moreover, the fact that random-like has such dropout robustness property justifies the need of avoiding complex co-adaption on the training test -- We would like to enforce the net to be random-like so that it doesn't overfit to any specific set of training examples with some complex co-adaption hidden there. 
%We theory shows that it is entirely possible for a network to perform good prediction when half of the nodes are dropped, and actually a random net and an observable drawn from the random net using our model has this dropout robustness. 
\Tnote{I don't really know how to expand this anymore. Not sure whether you will do more in the intro}
\fi 
%\subsection{Our regularization}

Thus our theory suggests that training should use dropout, since the hoped-for net has to be random-like. In addition it suggests that the training  should nudge the net --using a suitable regularizer--- in a direction where it becomes more consistent with the generative model described in the previous sections.  Now we derive such a regularizer;
%; and as already mentioned it is a form of the reconstruction idea of unsupervised learning. Also, 
as usual in such things, the derivation  will be intuitive, in contrast to 
the rigor of earlier sections. Furthermore, we do not have a closed form for the regularizer, only for its 
gradient (which suffices for training).

%We derive from our theory a simple regularization that seems to be a good alternatives to dropouts. 
%\Tnote{I think we should note that what follows are non-rigourous or hand-wavey approximations unlike other part of the paper?}

For simplicity  focus on a single layer and we use the notation in Section~\ref{sec:model}. Deriving a regularizer from a generative model 
requires thinking about how to change the model so as to improve the log likelihood of the data, so it is good to have differentiability as well as
nonzero probability for every data-point.  So we extend our model slightly to allow a guassian noise added on the observation: 
%\begin{equation}
$x = s_t(r(\alpha Wh)) + \xi$
%\end{equation}
where $s_t(\cdot)$ is the random function which samples the coordinate in $T$ and dropouts  values outside $T$, and $\xi$ is a small gaussian noise  with i.i.d entries with $\sigma^2$. 

The final form of the gradient of the log-likelihood via a series of approximation will be (where $\odot$ is entry-wise product of vectors) shown in Appendix~\ref{sec:der}:
\begin{equation}
\nabla_W \log p(x\mid h) \approx \left(x  - (r(Wh))\odot r'(Wh)\right)h^T \label{eqn:log-likelihood}
\end{equation}
We note that the resulting form is close to the expressions for contrastive divergence and the gradient of the reconstruction error used in auto-encoders. % which is expected. 
%Therefore, our generated $x$ is still close to $t$-sparse, and almost nonnegative. 

This gradient shows how to change model parameters to improve the generative model. Since our theory shows that the feedforward network shares the same weights with the generative network, one can incorporate the above regularizer into the training objective of feedforward neural network. Concretely, in our training of mutli-layer neural network, we add regularization for all of the layers simultaneously and equivalently, we update the parameters by 
\begin{equation}
W_{j} \leftarrow W_{j}  -\eta\left(\frac{\partial F}{\partial W} + \lambda_j\nabla_{W_j} \log p(\tilde{h}^{(j)}\mid h^{(j+1)}) \right)%\lambda_j G(h^{(j)}, h^{(j+1)})
\end{equation}
where $F$ is the training objective, and the gradient of log-likelihood is approximated by equation~\ref{eqn:log-likelihood}.  %$G(\cdot)$ is the approximate gradient of the log likelihood, and $\{\lambda_j\}$  are the regularization weights.


%\paragraph{Derivation of the approximation~\ref{eqn:log-likelihood}:}  We write the log likelihood of $x$ given $h$ under our model (with small gaussian noise added as discussed before), 
%$$\log \Pr[x\mid h] \propto\log \sum_{T: |T|=t} \exp(\|x-(r(\alpha Wh))_T\|^2/2\sigma^2)$$
%Note that since all the $T$'s of size $t$ are chosen with the same probability, here we have uniform sum of exponentials. In the
%spirit of Stochastic Gradient descent, we  do the naive approximation of simply picking a random subset $T$ to approximate the averaging over all $T$'s, and obtain
%$$R(W) = \log \Pr[x\mid h] \underset{\sim}{\propto}\|x-(r(\alpha Wh))_T\|^2$$
%where $T$ of size $t$ is picked uniformly at random.
%
%We take gradient of $R(W)$ over $W$ and obtain that $\frac{\partial R}{\partial W} \approx \left((x_T-r(Wh)_T)\odot r'(Wh)_T\right)h^T$ where $\odot$ denotes the entry-wise product of two vectors. Therefore taking expectation over the randomness of $T$ again, we obtain that 
%$$\nabla_W \log \Pr[x\mid h]  = \Exp_T\left[\frac{\partial R}{\partial W}\right] \approx \left(x  - (r(Wh))\odot r'(Wh)\right)h^T$$
%%\Tnote{Yingyu, could you please check whether this is what we used in the code? I am a bit too tired to get the gradient correctly..} \yingyu{we don't use sampling; otherwise yes}


%\Tnote{Maybe we could just cite the paper of Hinton for the connection? }




%To see the former, note that in training of RBM using contrastive divergence 
%\subsection{Connection to Contrastive Divergence}


%\label{sec:connection}


==> theoryapp_copy.tex <==
\section{Complete proofs for One-layer reversibility}\label{app:complet-one-layer}

\begin{proof}[Proof of Lemma~\ref{lem:beforerelu}] 
	%We fix the choice of $h$ and prove that~\eqref{eqn:reversible} is true for most of $W$ from~\eqref{eqn:prior}. This would implies that 
	We claim that it suffices to show  that w.h.p\footnote{We use w.h.p as a shorthand for ``with high probability'' in the rest of the paper. } over the choice of ($(W,h,x)$ the network is reversible (that is, ~\eqref{eqn:reversible} holds), 
	\begin{equation}
	\Pr_{x,h,W}\left[\textrm{equation~\eqref{eqn:reversible} holds}\right] \ge 1 - n^{10}\,.\label{eqn:joint-prob}
	\end{equation}
	Indeed, suppose~\eqref{eqn:joint-prob} is true, then using a standard Markov argument, we obtain  
	$$\Pr_{W}\left[\Pr_{x,h}\left[\textrm{equation~\eqref{eqn:reversible} holds} \mid W\right] > 1-n^{-5} \right]\ge 1 - n^{5},$$ as desired. 
	
	%Equation~(\ref{eqn:joint-prob}) is proven rigorously in Theorem~\ref{thm:single-technical} in supplementary materials, though here we give a proof sketch that demonstrates the idea. 
	Now we establish~\eqref{eqn:joint-prob}. Note that equation~\eqref{eqn:reversible} (and consequently statement~\eqref{eqn:joint-prob}) 
	holds for any positive scaling of $h,x$ simultaneously, since RELU has the property that $r(\beta z) = \beta \cdot r(z)$ for any $\beta \ge 0$ and any $z\in \mathbb{R}$.  Therefore WLOG we can choose a proper scaling of $h$ that is convenient to us. We assume $\|h\|_2^2 = k$. By assumption~\eqref{eqn:hdistribution}, we have that $|h|_{\infty}\le \widetilde{O}(\sqrt{\log k})$. 
	
	Define $\check{h} = \alpha W^Tx$. Similarly to~\eqref{eqn:hi}, we fix $i$ and expand the expression for $\check{h}_i$ by definition and obtain 
	$	\check{h}_i  = \alpha\sum_{j=1}^n W_{ji}x_j$. 
	%Suppose the random sampling function $s_t(\cdot)$ drops all the values outside support $T$, we can write $x_j$ as 
	Suppose $n_{\drop}$ has support $T$.  Then we can write $x_j$ as 
	\begin{align}
	x_j  &=  \relu(\sum_{\ell=1}^m W_{j\ell} h_{\ell}) \cdot n_{\drop,j}=  \relu(W_{ji} h_i + \eta_j)\cdot \mathbf{1}_{j\in T} \,,\label{eqn:eqn29}
	\end{align}
	where $\eta_j \triangleq \sum_{\ell\neq j}W_{j\ell}h_{\ell}$. Though $\relu(\cdot)$ is nonlinear, it is piece-wise linear and more importantly still Lipschitz. Therefore intuitively, RHS of~\eqref{eqn:eqn29} can be ``linearized" by approximating 
	$	\relu(W_{ji}h_i + \eta_j) $ by $\mathbf{1}_{\eta_j > 0}\cdot \left(W_{ji}h_i + \relu(\eta_j)\right)$. 
	%	\begin{equation}
	%	\relu(W_{ji}h_i + \eta_j) \approx  \mathbf{1}_{\eta_j > 0}\cdot W_{ji}h_i + \relu(\eta_j) \label{eqn:approx}
	%	\end{equation}
	Note that this approximation is not accurate only when $|\eta_j|\le |W_{ji}h_i|$, which happens with relatively small probability, since $\eta_j$ typically dominates $W_{ji}h_{i}$ in magnitude. %(note that  while $W_{ji}h_i$ is only one term while $\eta_j = \sum_{\ell\ne i}W_{j\ell}h_{\ell}$ is a sum, therefore the latter typically dominates the former).
	
	Using the intuition above, we can formally calculate the expectation of $W_{ji}x_j$ via a slightly tighter and more sophisticated argument: Conditioned on $h$, we have $W_{ji}\sim\mathcal{N}(0,1)$ and  $\eta_j = \sum_{\ell\neq j}W_{j\ell}h_{\ell} \sim \mathcal{N}(0,\sigma^2)$ with $\sigma^2 = \|h\|^2 - h_j^2 = k - h_j^2 \ge \Omega(k)$. Therefore we have $\log \sigma = \frac{1}{2}\log (\Omega(k)) \ge h_j$ and then by Lemma~\ref{lem:exp} ($W_{ji}$ here corresponds to $w$ in Lemma~\ref{lem:exp}, $\eta_j$ to $\xi$ and $h_j$ to $h$), we have 
	$
	\Exp[W_{ji}x_j \mid h] = \Exp[W_{ji}r(W_{ji}h_j + \eta_j) \mid h] = \frac{1}{2} h_i \pm \widetilde{O}(1/k^{3/2})\nonumber
	$. 
	
	It follows that 
	\begin{equation}
	\Exp[\check{h}_i\vert h,T] = \sum_{j\in T} \Exp[W_{ji}r(W_{ji}h_j + \eta_j) \mid h] = \frac{\alpha |T|}{2}  h_i \pm \widetilde{O}(\alpha t/k^{3/2})\nonumber
	\end{equation}
	
	Taking expectation over the choice of $T$ we obtain that \begin{equation}
	\Exp[\check{h}_i\vert h] = \frac{\alpha t}{2}  h_i \pm \widetilde{O}(\alpha n/k^{3/2}) = h_i \pm \widetilde{O}(1/(k^{3/2})) \label{eqn:expectation}
	\end{equation} . (Recall that $t = \rho n$ and $\alpha = 2/(\rho n)$. Similarly, the variance of $\check{h}_i\vert h$ can be bounded by 
	$\Var[\check{h}_i \vert h] = O(k/t)$ (see Claim~\ref{lem:app:var}). Therefore we expect that $\check{h}_i$ concentrate around its mean with fluctuation $\pm O(\sqrt{k/t})$. Indeed, by 
	%	
	%	Equation~(\ref{eqn:approx}) implies that $W_{ji}x_j$ can be written approximately as 
	%	\begin{align}
	%	W_{ji}x_j % &= W_{ji}\cdot \relu(\sum_{\ell}\cdot W_{j\ell}x_{\ell}) \cdot \mathbf{1}_{j\in T} \nonumber\\
	%	& \approx \underbrace{W_{ji}^2h_i \cdot \mathbf{1}_{\eta_j > 0}\cdot \mathbf{1}_{j\in T}}_{\textrm{signal: } \mu_j'}  +\underbrace{W_{ji}r(\eta_j)\cdot \mathbf{1}_{j\in T} }_{\textrm{noise: } \eta_j'} 
	%	\end{align}
	%Though here we have a more complicated formula than~\eqref{eqn:wjihatxj}, actually the same intuition applies: when taking sum of $W_{ji}x_j$ over $j$, $u_j'$ contributes to the signal term, while the sum of $W_{ji}r(\eta_j')$ attenuates due to cancellation (note that it is still mean zero due to the fact $W_{ji}$ is mean zero and independent with $r(\eta_j')$. %has mean zero and contributes the variance, and we obtain that 
	by concentration inequality, we can prove (see Lemma~\ref{lem:concentration} in Section~\ref{app:complet-one-layer}) that actually $\check{h}_i\mid h$ is sub-Gaussian, and therefore  conditioned on $h$, with high probability ($1-n^{-10}$) we have $|\check{h}_i -  h_i| \le \widetilde{O}((\sqrt{k/t}+ 1/k^{3/2})$, where the first term account for the variance and the second is due to the bias (difference between $\Exp[\check{h}_i]$ and $h_i$). 
	%$$\Pr\left[|\check{h}_i -  h_i| \ge \widetilde{\Omega}((\sqrt{k/t}+ 1/(tk^{3/2}))\mid h\right] \le n^{-10}\,.$$
	
	Noting that $k < t < k^2$ and therefore $1/k^{3/2}$ is dominated by $\sqrt{k/t}$, take expectation over $h$, we obtain that $\Pr\left[|\check{h}_i -  h_i| \ge \widetilde{\Omega}(\sqrt{k/t})\right] \le n^{-10}$. Taking union bound over all $i\in [n]$, we obtain that with high probability, $\|\check{h} - h\|_{\infty} \le \widetilde{O}(\sqrt{k/t})$.  Recall that $\|h\|$ was assumed to be equal $k$ without loss of generality. Hence we obtain that $\|\check{h} - h\|_{\infty} \le \widetilde{O}(\sqrt{1/t})\|h\|$ as desired. 
	
	
	%Therefore we have $\check{h}_i \approx \alpha \sum_{j=1}^n(u_j'+\eta_j') = \alpha Ch_i + \alpha R' $, 
	%	where $C$ is a scaling constant which depends essentially on the size of $T$, while $R'$ corresponds to the noise which is a sum of random like numbers. A careful computation can be done and we will show that when $k \ll t$, %($k$ and $t$ are the sparsity of $h$ and $x$), 
	%	$R'$ is dominated by the signal term $Ch_i$. Choosing $\alpha = 1/C$, we can show that for some small $\epsilon$, for any $i$, 
	%	$|\check{h}_i - h_i| \le \epsilon$
	%	and therefore we have approximate reversibility, and $\alpha \check{h}$ actually is close to $h$ in euclidean norm: $\|\check{h} - h\|\le \epsilon \sqrt{n}$. 
	%where the noise will shown to be dominated by $h_i$ for $h_i$ being bounded away from 0. Choosing a proper scaling of $\alpha$, we obtain that $\alpha \check{h}_i = h_i \pm \epsilon$ for some small $\epsilon$. In vector notation, we obtain that 
	%$$|\alpha \check{h} - h|_{\infty} \lesssim \epsilon, \textrm{ and } \|\alpha \check{h} - h \| \le \epsilon \sqrt{m}$$
	
	%\Tnote{Require a bit edit below}
	
	%	To finish, we show that taking another rectifier linear on $\alpha\check{h}$ will further reduce the noise. Suppose $h$ has support $K$ of size $k$. We choose $\tilde{b} = -\epsilon\mathbf{1}$, and let $\tilde{h}  =\relu(\check{h} +  \tilde{b}) = \relu(W^Th + \tilde{b})$, then we obtain that for $i\not \in K$,  $\tilde{h}_i  = r(\check{h}_i ) = r(h_i\pm \epsilon + b) = 0$. Therefore, for those $i\not\in K$, there is no loss $\tilde{h}_i = h_i  = 0$. Moreover, this addition nonlinear operation doesn't incur more loss on $K$ either -- for any $i$, it is guaranteed that $|\tilde{h}_i - h_i| \le |\tilde{h_i}-\check{h}_i|+|\check{h}_i- h_i|\le 2\epsilon$. Therefore the total error between $\tilde{h}$ and $h$ in euclidean distance can be bounded by %Therefore using rectifier linear with a small shift $b \approx \epsilon$, the resulting $\tilde{h}$ is exactly equal to 0 when $h_i = 0$, and for $h_i \neq 0$, it only introduce at most another small error $\epsilon$. Therefore then we have that 
	%	%\begin{equation}
	%	$\|\tilde{h} - h\| = \|r(\alpha W^Tx) - h\|\le \epsilon\sqrt{k} $
\end{proof}

%
%%For simplicity of the notation, Suppose we have hidden layer $h\in \mathbb{R}^m$ and observable $x\in \mathbb{R}^n$. We assume that the observable $x$ is generated by $x = s_t(\relu(Wh))$ where $W$ is the weight matrix and $\relu$ is the rectifier linear function and $s_t(\cdot)$ is a random sampling function (as specified above).
%%In this section, \textquotedblleft random-like\textquotedblright~ means that $W\in\mathbb{R}^{n\times m}$ is a random gaussian matrix with each entry independently drawn from $\mathcal{N}(0,1)$. We consider the situation when $s_t(\cdot)$ basically picks a random subset $T$ of size $t$ and zeroes out the entries outside $T$. 
%
%%Given the observable $x$, we run the network in feed-forward direction with the same weight $W$ and obtain $$\tilde{h} = r(\alpha W^Tx - b\mathbf{1})$$ where $\alpha$ is a scaling constant and $b\mathbf{1}$ is the offset vector. We prove the following: 
%Here we use slight different notation and scaling as in Section~\ref{sec:model} for the ease of exposition. %We use the same n. otation as in Section~\ref{sec:model}. 
%We recall that $W\in \mathbb{R}^{n\times m}$ is assumed to be drawn from prior, 
%\begin{equation}
%W_{ij}\sim \mathcal{N}(0,1) \nonumber %\label{eqn:prior}
%\end{equation}
%In the following technical main theorem, we assume that conditioned on a fixed $h$ while $W$ is random. We define the generative model without the scaling in this section, that is,  $x$ is generated from 
%$$x = s_t(r(Wh))$$
%and we define the feedforward calculation with the scaling $\alpha$, that is, $\tilde{h}$ is defined as 
%$$\tilde{h} = r(\alpha W^Tx + b)$$
%
%Note that since $\alpha r(x) = r(x)$ for any $x$ and positive $\alpha$. This model is equivalent to the model in Section~\ref{sec:model} perse. 
%where $W_{ij}$ are independent with each other. 
%Then we have the following theorem
%Then we assume that $h$ has a distribution $\mathcal{D}_h$ over $k$-sparse vectors, 
%We assume the hidden variable $h$ has a $D_h$ over the $k$-sparse vectors. Technically, we assume when $h\sim D_h$, 
%\begin{eqnarray}
%|h|_0 \le k \textrm{ and } |h|_{\infty} \ll \|h\|\quad \textrm{a.s.} \nonumber %\label{eqn:hdistribution}
%\end{eqnarray}
%\begin{theorem}[Reversibility]\label{thm:single-technical}
%	For  $k <  t\le k^2$, and any fixed $h\in \mathbb{R}^m$ with $|h|_0 \le k$ and $\|h\|_2 =\Theta(\sqrt{k})$ and $|h|_{\infty}\le \tilO(1)$, for $\alpha = \frac{2}{t}$ and some $b$ with $b = -\epsilon\mathbf{1}$ where $\epsilon = \tilOmega(\sqrt{k/t})$, with high probability over the randomness of $W$, $\tilde{h}$ satisfies that $$\|h-\tilde{h}\|^2\le \tilO\left(\frac{k}{t}\right)\|h\|^2$$ %for $\hat{h} = \alpha W^Tx$  with the scaling constant $\alpha = \frac{2}{s}$, we have that $|\hat{h}-h|_{\infty} \le \tilO\left(\frac{\|h\|}{\sqrt{s}}
%	%\right)+ \tilO\left(\frac{1}{\|h\|^3}\right)$
%\end{theorem} 
%%The proof of the theorem uses the following lemma which prove that $\hat{h} = r(Wh)$ is close to $h$ in $\ell_{\infty}$ norm.
%\begin{lemma}\label{lem:single-reversibility}
%	%For any fixed $h$ with $|h|_0 = k$ and $\|h\|_{\infty}\ll \|h\|_2 =\Theta(\sqrt{k})$, with high probability over the randomness of $W$, for $\hat{h} = \alpha W^Tx$  with the scaling constant $\alpha = \frac{2}{t}$, 
%	Under the same condition as in Theorem~\ref{thm:single-technical}, we have that $|\hat{h}-h|_{\infty} \le \tilO\left(\sqrt{k/t}\right)$. Therefore we observe that $r(\hat{h}_i - \epsilon) = 0$ when $h_i = 0$ and moreover when $|r(\hat{h}_i - \epsilon) - h_i| \le 2\epsilon$ when $h_i\neq 0$. Let $K$ be the support of $h_i$. We have that $|K|=k$, and $\|\tilde{h} - h\|^2 = \sum_{i=1}^m |r(\hat{h}_i - \epsilon) - h_i|^2  = \sum_{i\in K} |r(\hat{h}_i - \epsilon) - h_i|^2 \le k\epsilon^2$. Plugging in $\epsilon = \tilO\left(\sqrt{k/t}\right)$ we obtain the desired result. 
%\end{lemma} 
%
%\begin{proof}[Proof of Theorem~\ref{thm:single-technical}]
%	Note that by Lemma~\ref{lem:single-reversibility}, we have that whp  $|\hat{h}_i - h_i| \le \epsilon$ for $\epsilon = \tilO\left(\sqrt{k/t}\right)$
%\end{proof}

%\begin{proof}[Proof of Lemma~\ref{lem:single-reversibility}]
%	We fix the choice of function $s_t(\cdot)$ by assuming  $s(x) = [x_T,0]$ for some fixed set $T$ of size $t$. Throughout the rest of the proof, we fix an index $i\in [m]$, and we are going to prove that with high probability $|\hat{h}_i - h_i |\le \tilO\left(\sqrt{k/t}\right)$. Therefore taking union bound we will obtain the desired result. 
%	
%	By definition, $\hat{h}_i = \frac{2}{t}\sum_{j\in [n]}W_{ji}x_j $ where $x_j = \relu((Wh)_j) = \relu(\sum_{t\in [m]}W_{jt}h_t)$ for $j\in T$ and $x_j=0$ for $j\not\in T$. Therefore, for $j\in T$, we define $Z_j = W_{ji}x_j$ which can be written as
%	$$Z_j = W_{ji}x_j = W_{ji}\relu(W_{ji}h_i + \sum_{t\neq i}W_{jt}h_t)$$
%	Note that $\sum_{t\neq i}W_{jt}h_t$ has a gaussian distribution with variance $\sigma^2  = \|h\|^2 - h_i^2$,  and $W_{ji}$ is from standard normal distribution, so they meet the form of Lemma~\ref{lem:exp}. Therefore by Lemma~\ref{lem:exp}, we obtain that $\Exp[Z_j] = \Exp[W_{ji}x_j]= \frac{h_i}{2} \pm \tilO(1/\|h\|^3)$. Moreover, since $W_{ji}$ and $x_j$ are subgaussian random variables, we have that $\|W_{ji}\|_{\psi_2} = 1$ and $\psinorm{x_j}{2}\le \|h\|$. Then we have that $W_{ji}x_j$ is sub-exponential random variables, that is, $\psinorm{W_{ji}x_j}{1}\le O(\|h\|)$. That is, $Z_j$ has $\psi_1$ orlicz norm at most $O(\|h\|)$ and moreover by lemma~\ref{lem:psi-norm-mean-shift}, $\psinorm{Z_j-\E[Z_j]}{1} \le O(\|h\|)$. Finally we note that $Z_j$'s are independent random variables and therefore we are ready to apply bernstein inequalities for sub-exponential random variables (Theorem~\ref{thm:berstein-psi1}) and obtain that for some universal constant $c$, 
%	
%	\begin{equation*}
%	\Pr\left[\left|\sum_{j\in T} Z_j - \Exp\left[\sum_{j\in T} Z_j\right]\right| > c\sqrt{|T|}\|h\|\log n\right] \le n^{-10}
%	\end{equation*}
%	
%	Recall the definition of $Z_j = W_{ji}x_j$, $\hat{h_i} = \sum_{j\in T}Z_j$, and the fact that $\Exp[Z_j] = h_i/2 \pm \tilO(1/\|h\|^3)$, we obtain that with high probability over the randomness of $W$, $$\|\hat{h}_i - h_i\|\le \tilO\left(\frac{\|h\|}{\sqrt{t}}
%	\right)+ \tilO\left(\frac{1}{\|h\|^3}\right)$$
%	
%	Note that under our assumption we have that $\frac{1}{\|h\|^3}\le O(\frac{\|h\|}{\sqrt{t}})$ when $\|h\|^4  =\Theta(k^2)\ge t$. Therefore the proof is complete. 
%	
%	
%	
%	%Moreover, by Lemma~\ref{lem:exp} gain, the variance of $W_{ji}x_j$ can be simply bounded by $\Exp[W_{ij}^2x_j^2]\le 3h_i^2 + \|h\|^2 - h_i^2 = \|h\|^2 + 2h_i^2$. 
%	%	\begin{align*}
%	%	\mathbb{V}[W_{ji}x_j]&\le \Exp[W_{ji}^2x_j^2]\le \Exp\left[W_{ji}^2(W_{ji}h_i + \sum_{t\neq i}W_{jt}h_t)^2\right] \\
%	%	& = \Exp[W_{ji}^2]
%	%	\end{align*}
%	
%	%The proof simply follows f$rom the fact that 
%\end{proof}
\begin{proof}[Proof of Theorem~\ref{thm:dropout}]
	%Almost the same as Theorem~\ref{thm:single}, 
	Recall that in the generative model already many bits are dropped, 
	% in the generative direction, 
	and nevertheless the feedforward direction maps it back to $h$. Thus dropping some more bits in $x$ doesn't make much difference. Concretely, we note that $x^{\drop}$ has the same distribution as $s_{t/2}(r(\alpha Wh))$. Therefore invoking Theorem~\ref{thm:single} with $t$ being replaced by $t/2$, we obtain that there exists $b'$ such that $\|r(2W^Tx^{\textrm{drop}} + b')- h\|^2 \le \tilO(k/t)\cdot \|h\|$.%-- the nature of our generative model essentially captures the dropout. 
	%\Tnote{The proof requires a slight change of notation}
\end{proof}

\begin{lemma}\label{lem:concentration} Under the same setting as Theorem~\ref{thm:single}, let $\check{h} = \alpha W^Th$. Then we have
	$$\Pr\left[|\check{h}_i -  h_i| \ge \widetilde{\Omega}((\sqrt{k/t}+ 1/k^{3/2})\mid h\right] \le n^{-10}$$
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:concentration}]
		Recall that $\check{h}_i =  \sum_{j\in T} \alpha W_{ji}r(W_{ji}h_j + \eta_j)$. For convenience of notation, we condition on the randomness $h$ and $T$ and only consider the randomness of $W$ implicitly and omit the conditioning notation. Let $Z_j$ be the random variable $\alpha W_{ji}x_j = \alpha W_{ji}r(W_{ji}h_j + \eta_j)$. Therefore $Z_j$ are independent random variables (conditioned on $h$ and $T$). Our plan is to show that $Z_j$ has bounded Orlicz norm and therefore $\check{h}_i = \sum_j Z_j $ concentrates around its mean. 
%		
%		
%		We apply random 
%		\begin{equation}
%		\Exp[\check{h}_i\vert h,T] = \sum_{j\in T} \Exp[W_{ji}r(W_{ji}h_j + \eta_j) \mid h] = \frac{\alpha |T|}{2}  h_i \pm \widetilde{O}(\alpha n/k^{3/2})\nonumber
%		\end{equation}
%		
%		Taking expectation over the choice of $T$ we obtain that $\Exp[\check{h}_i\vert h] = \frac{\alpha t}{2}  h_i \pm \widetilde{O}(\alpha n/k^{3/2}) = h_i \pm \widetilde{O}(1/(tk^{3/2})) $. (Recall that $t = \rho n$ and $\alpha = 2/(\rho n)$. Moreover the variance of $\check{h}_i\vert h$ can be bounded by 
%		\begin{equation}
%		\Var[\check{h}_i \vert h] = \Exp_T\left[\sum_{j\in T}\alpha^2 \Var[W_{ji}x_j\vert h]\right] \le \alpha^2 t\cdot O(k) = O(k/t),  \nonumber
%		\end{equation}
%		
%		where we used Cauchy-Schwartz inequality, that is,  $\Var[W_{ji}x_j\vert h]  \le \Exp[W_{ji}^2x_j]^2\vert h] \le \Exp[W_{ji}^4\vert h]^{1/2}\Exp[x_j^4\vert h]^{1/2}\le O(k)$ (a tighter calculation can be found in Lemma~\ref{lem:exp}). 
		%	
		%	Equation~(\ref{eqn:approx}) implies that $W_{ji}x_j$ can be written approximately as 
		%	\begin{align}
		%	W_{ji}x_j % &= W_{ji}\cdot \relu(\sum_{\ell}\cdot W_{j\ell}x_{\ell}) \cdot \mathbf{1}_{j\in T} \nonumber\\
		%	& \approx \underbrace{W_{ji}^2h_i \cdot \mathbf{1}_{\eta_j > 0}\cdot \mathbf{1}_{j\in T}}_{\textrm{signal: } \mu_j'}  +\underbrace{W_{ji}r(\eta_j)\cdot \mathbf{1}_{j\in T} }_{\textrm{noise: } \eta_j'} 
		%	\end{align}
		
		%Though here we have a more complicated formula than~\eqref{eqn:wjihatxj}, actually the same intuition applies: when taking sum of $W_{ji}x_j$ over $j$, $u_j'$ contributes to the signal term, while the sum of $W_{ji}r(\eta_j')$ attenuates due to cancellation (note that it is still mean zero due to the fact $W_{ji}$ is mean zero and independent with $r(\eta_j')$. %has mean zero and contributes the variance, and we obtain that 
%		
%		By concentration inequality, we can prove (see Lemma~\ref{lem:concentration} in Section~\ref{app:complet-one-layer}) that actually $\check{h}_i$ is sub-Gaussian, and therefore we have 
%		
%	We fix the choice of function $s_t(\cdot)$ by assuming  $s(x) = [x_T,0]$ for some fixed set $T$ of size $t$. Throughout the rest of the proof, we fix an index $i\in [m]$, and we are going to prove that with high probability $|\hat{h}_i - h_i |\le \tilO\left(\sqrt{k/t}\right)$. Therefore taking union bound we will obtain the desired result. 
%%	
%	By definition, $\hat{h}_i = \frac{2}{t}\sum_{j\in [n]}W_{ji}x_j $ where $x_j = \relu((Wh)_j) = \relu(\sum_{t\in [m]}W_{jt}h_t)$ for $j\in T$ and $x_j=0$ for $j\not\in T$. Therefore, for $j\in T$, we define $Z_j = W_{ji}x_j$ which can be written as
%	$$Z_j = W_{ji}x_j = W_{ji}\relu(W_{ji}h_i + \sum_{t\neq i}W_{jt}h_t)$$
%	Note that $\sum_{t\neq i}W_{jt}h_t$ has a gaussian distribution with variance $\sigma^2  = \|h\|^2 - h_i^2$,  and $W_{ji}$ is from standard normal distribution, so they meet the form of Lemma~\ref{lem:exp}. 
	
%	Recall as shown in the proof of Theorem~\ref{thm:single}, by Lemma~\ref{lem:exp}, we obtain that $\Exp[Z_j] = \Exp[W_{ji}x_j]= \alpha h_i/2 \pm \tilO(1/k^{3/2})$.
 Since $W_{ji}$ and $x_j$ are Gaussian random variables with variance 1 and $\|h\|=  \sqrt{k}$, we have that $\|W_{ji}\|_{\psi_2} = 1$ and $\psinorm{x_j}{2}\le \sqrt{k}$. This implies that $W_{ji}x_j$ is sub-exponential random variables, that is, $\psinorm{W_{ji}x_j}{1}\le O(\sqrt{k})$. That is, $Z_j$ has $\psi_1$ orlicz norm at most $O(\alpha \sqrt{k})$. Moreover by Lemma~\ref{lem:psi-norm-mean-shift}, we have that $\psinorm{Z_j-\E[Z_j]}{1} \le O(\alpha \sqrt{k})$. %Finally we note that $Z_j$'s are independent random variables and therefore 
 Then we are ready to apply bernstein inequalities for sub-exponential random variables (Theorem~\ref{thm:berstein-psi1}) and obtain that for some universal constant $c$, 
	
	\begin{equation*}
		\Pr\left[\left|\sum_{j\in T} Z_j - \Exp\left[\sum_{j\in T} Z_j\right]\right| > c\sqrt{|T|}\alpha \sqrt{k}\log n\right] \le n^{-10}\,.
	\end{equation*}
	
	Equivalently, w obtain that 
	
		\begin{equation*}
		\Pr\left[\left|\check{h}_i - \Exp\left[\check{h}_i\right]\right| > c\sqrt{|T|k/t^2}\log n\mid h,T\right] \le n^{-10}\,.
		\end{equation*}
		
		Note that with high probability, $|T| = (1\pm o(1)) t$. Therefore taking expectation over $T$ and taking union bound over $i\in [n]$ we obtain that for some absolute constant $c$,  
	\begin{equation*}
	\Pr\left[\forall i\in [n], \left|\check{h}_i - \Exp\left[\check{h}_i\right]\right| > c\sqrt{k/t}\log n\mid h\right] \le n^{-8}\,.
	\end{equation*}
	
	Finally note that as shown in the proof of Theorem~\ref{thm:single}, we have $\Exp[\check{h}_i\mid h] = h_i \pm 1/k^{3/2}$. Combining with the equation above we get the desired result. 
	%Recall the definition of $Z_j = W_{ji}x_j$, $\hat{h_i} = \sum_{j\in T}Z_j$, and the fact that $\Exp[Z_j] = h_i/2 \pm \tilO(1/\|h\|^3)$, we obtain that with high probability over the randomness of $W$, $$\|\hat{h}_i - h_i\|\le \tilO\left(\frac{\|h\|}{\sqrt{t}}
%	\right)+ \tilO\left(\frac{1}{\|h\|^3}\right)$$
	
%	Note that under our assumption we have that $\frac{1}{\|h\|^3}\le O(\frac{\|h\|}{\sqrt{t}})$ when $\|h\|^4  =\Theta(k^2)\ge t$. Therefore the proof is complete. 
	
	
	
	%Moreover, by Lemma~\ref{lem:exp} gain, the variance of $W_{ji}x_j$ can be simply bounded by $\Exp[W_{ij}^2x_j^2]\le 3h_i^2 + \|h\|^2 - h_i^2 = \|h\|^2 + 2h_i^2$. 
	%	\begin{align*}
	%	\mathbb{V}[W_{ji}x_j]&\le \Exp[W_{ji}^2x_j^2]\le \Exp\left[W_{ji}^2(W_{ji}h_i + \sum_{t\neq i}W_{jt}h_t)^2\right] \\
	%	& = \Exp[W_{ji}^2]
	%	\end{align*}
	
	%The proof simply follows f$rom the fact that 
\end{proof}

\begin{claim}\label{lem:app:var}
	Under the same setting as in the proof of Theorem~\ref{thm:single}. The variance of $\check{h}_i$ can be bounded by 
	\begin{equation}
	\Var[\check{h}_i \vert h]  \le O(k/t) \nonumber
	\end{equation}
\end{claim}
\begin{proof}
	Using Cauchy-Schwartz inequality we obtain 
	
	\begin{align*}
	\Var[W_{ji}x_j\vert h]  & \le \Exp[W_{ji}^2x_j]^2\vert h] \\
	& \le \Exp[W_{ji}^4\vert h]^{1/2}\Exp[x_j^4\vert h]^{1/2}\le O(k)
	\end{align*}
	It follows that 
	\begin{align*}
	\Var[\check{h}_i \vert h] & = \Exp_T\left[\sum_{j\in T}\alpha^2 \Var[W_{ji}x_j\vert h]\right] \le \alpha^2 t\cdot O(k) = O(k/t),  \nonumber
	\end{align*}
	
	%where we used Cauchy-Schwartz inequality, that is,  $\Var[W_{ji}x_j\vert h]  \le \Exp[W_{ji}^2x_j]^2\vert h] \le \Exp[W_{ji}^4\vert h]^{1/2}\Exp[x_j^4\vert h]^{1/2}\le O(k)$ 
	
	We note that a tighter calculation of the variance can be obtained using Lemma~\ref{lem:exp}). 
\end{proof}
\section{Auxiliary lemmas for one layer model }\label{sec:onelayertechnical}

We need a series of lemmas for the one layer model, which will be further used in the proof of two layers and three layers result. %Throughout this section, we use the same setting in Section~\ref{sec:onelayertechnical}. 

As argued earlier, the particular scaling of the distribution of $h$ is not important, and we can assume WLOG that $\|h\|^2 = k$. Throughout this section, we assume that for $h\sim D_h$, 
\begin{eqnarray}
h \in \mathbb{R}_{\ge 0}^n, \quad |h|_0 \le k \, ,\,\|h\| =k\,,\, \textrm{ and }\, |h|_{\infty} \le O(\sqrt{\log N})\quad \textrm{almost surely} \label{eqn:scaledassumption}
\end{eqnarray}
%\Tnote{To check the notation}
\begin{lemma}\label{lem:exp}
	Suppose $w\in \mathcal{N}(0,1)$ and $\xi\sim \mathcal{N}(0,\sigma^2)$ are two independent variables. For $\sigma = \Omega(1)$ and $0\le h\le \log(\sigma)$, we have that $\Exp\left[w\cdot \relu(wh+ \xi)\right] = \frac{h}{2} \pm \tilO(1/\sigma^3)$ and $\Exp[w^2\cdot \relu(wh+ \xi)^2] \le 3h^2+\sigma^2$. 
\end{lemma} 

\begin{proof}
	Let $\phi(x) =\frac{1}{\sigma\sqrt{2\pi}}\exp(-\frac{x^2}{2\sigma^2})$ be the density function for random variable $\xi$. Let $C_1 = \Exp[|\xi|/\sigma] =\frac{2}{\sigma}\int_{0}^{\infty} \phi(x)xdx$. We start by calculating $\Exp\left[\relu(wh+\xi)\mid w\right]$ as follows: 
	
	\begin{align*}
	\Exp\left[w\cdot \relu(wh+\xi)\mid w\right] &= w\int_{-wh}^{\infty}\phi(x)(wh+x)dx \\
	& = w\int_{0}^{\infty}\phi(x)(wh+x)dx + w\int_{-wh}^{0}\phi(x)(wh+x)dx \\
	& = \frac{C_1\sigma w}{2} + \frac{w^2h}{2}  + \underbrace{w\int_{0}^{wh}\phi(y)(wh-y)dy}_{G(w)}\\
	\end{align*}
	Therefore we have that 
	\begin{align*}
	\Exp\left[\Exp\left[w\cdot \relu(wh+\xi)\mid w\right]\right] & %= \int_{-wh}^{\infty}\phi(x)(wh+x)dx \\
	%& = \int_{0}^{\infty}\phi(x)(wh+x)dx + \int_{-wh}^{0}\phi(x)(wh+x)dx \\
	= \frac{h}{2}  + \Exp[G(w)]
	\end{align*}
	Thus it remains to understand $G(w)$ and bound its expectation. We calculate the derivative of $G(w)$: We have that $G(w)$ can be written as 
	
	$$G(w) = w^2h\int_{0}^{wh}\phi(y)dy - w\int_{0}^{wh}\phi(y)ydy$$ 
	and its derivative is 
	\begin{align*}
	G(w)' & = 2wh\int_{0}^{wh}\phi(y)dy + w^2h^2\phi(wh) - \int_{0}^{wh}\phi(y)ydy - w^2h^2\phi(wh) \\
	& = 2wh\int_{0}^{wh}\phi(y)dy  - \int_{0}^{wh}\phi(y)ydy 
	\end{align*}
	The it follows that 
	\begin{align*}
	G(w)'' %& = 2wh\int_{0}^{wh}\phi(y)dy + w^2h^2\phi(wh) - \int_{0}^{wh}\phi(y)ydy - w^2h^2\phi(wh) \\
	& = 2h\int_{0}^{wh}\phi(y)dy + 2wh^2\phi(wh)  - wh^2\phi(wh) \\
	& = 2h\int_{0}^{wh}\phi(y)dy + wh^2\phi(wh)  
	\end{align*}
	Moreover, we can get the third derivative and forth one 
	\begin{align*}
	G(w)''' %& = 2wh\int_{0}^{wh}\phi(y)dy + w^2h^2\phi(wh) - \int_{0}^{wh}\phi(y)ydy - w^2h^2\phi(wh) \\
	%& = 2h\int_{0}^{wh}\phi(y)dy + 2wh^2\phi(wh)  - wh^2\phi(wh) \\
	& = 3h^2\phi(wh)+ wh^3\phi'(wh)  
	\end{align*}
	and 
	\begin{align*}
	G(w)^{(4)} %& = 2wh\int_{0}^{wh}\phi(y)dy + w^2h^2\phi(wh) - \int_{0}^{wh}\phi(y)ydy - w^2h^2\phi(wh) \\
	%& = 2h\int_{0}^{wh}\phi(y)dy + 2wh^2\phi(wh)  - wh^2\phi(wh) \\
	& = 4h^3\phi'(wh)+ wh^4\phi''(wh)
	\end{align*}
	Therefore for $h \le 10\log(\sigma)$ and $w$ with $|w|\le 10\log(\sigma)$, using the fact that $\phi'(wh) = \frac{1}{\sigma\sqrt{2\pi}}\exp(-\frac{w^2h^2}{2\sigma^2})\frac{wh}{\sigma^2}\le \frac{2wh}{\sigma^3\sqrt{2\pi}}$ and similarly, $\phi''(wh) \le \frac{1}{\sigma^3\sqrt{2\pi}}$. It follows that $G(w)^{(4)}\le O(\frac{wh^4}{\sigma^3})$ for any $w\le 10\log(\sigma)$. 
	
	Now we are ready to bound $\Exp[G(w)]$: By Taylor expansion at point 0,  we have that $G(w) = \frac{h^2\phi(0)}{2}w^3 + \frac{G(\zeta)^{(4)}}{24}w^4$ for some $\zeta$ between $0$ and $w$. It follows that for $|w|\le 10\log(\sigma)$, $|G(w) - \frac{h^2\phi(0)}{2}w^3|\le \tilO(1/\sigma^3)$, and therefore we obtain that 
\begin{align*}
	\left|\Exp\left[G(w)\mid |w|\le 10\log \sigma\right] - \Exp\left[\frac{h^2\phi(0)}{2}w^3\mid  |w|\le 10\log \sigma\right]\right| & \le \Exp\left[\left|G(w)- \frac{h^2\phi(0)}{2}w^3\right|\mid |w|\le 10\log \sigma\right]  \\
	& \	\le \tilO(1/\sigma^3)
\end{align*}
	

	Since $w| |w|\le 10\log \sigma$ is symmetric,  we have $\Exp\left[\frac{h^2\phi(0)}{2}w^3\mid  |w|\le 10\log \sigma\right] =0$, and it follows that $\Exp[G(w)\mid |w|\le 10\log \sigma] \le \tilO(1/\sigma^3)$. Moreover, note that $|G(w)|\le O(w^3h^2)\le O(\log^2\sigma w^3)$, then we have that 
	$$\Exp[G(w)\mid |w|\ge 10\log\sigma] \Pr[|w|\ge 10\log\sigma] \le \sigma^{-4}\int_{|w|\ge 10\log\sigma}O(\log^2\sigma w^3) \exp(-w^2/2)dw\le O(1/\sigma^3)$$
	Therefore altogether we obtain 
	\begin{align*}
	\Exp[G(w)] &=\Exp[G(w)\mid |w|\ge 10\log\sigma ] \Pr[|w|\ge 10\log\sigma]+\Exp[G(w)\mid |w|\le 10\log \sigma]\Pr[ |w|\le 10\log \sigma] \\
	& = \tilO(1/\sigma^3) + O(1/\sigma^3) = \tilO(1/\sigma^3). 
	\end{align*}
	
	Finally we bound the variance of $w\cdot\relu(wh+\xi)$. We have that 
	
	\begin{align*}
	\Exp[w^2\cdot\relu(wh+\xi)^2] & \le \Exp[w^2\cdot(wh+\xi)^2]  = h^2\Exp[w^4] + \Exp[w^2]\Exp[\xi^2] = 3h^2 + \sigma^2\,.\\
	\end{align*}
	as desired. 
	
\end{proof}


\begin{lemma}\label{lem:two-correlation}
	For any $a,b\ge 0$ with $a,b\le 5\log \sigma$ and random variable $u,v\sim \mathcal{N}(0,1)$ and $\xi\in \mathcal{N}(0,\sigma^2)$, we have that
	%$\Exp[uv\cdot\relu(au+bv+\xi)^2] =  ab \pm \tilO(1/\sigma)$, and moreover, 
	$\left|\Exp[uv\cdot\relu(au+bv+\xi)^2]  - \Exp[u\relu(au+bv+\xi)]\Exp[v\relu(au+bv+\xi)]\right|=  \tilO(1)$. 
	
\end{lemma}

\begin{proof}
	Let $t = \sqrt{a^2+b^2}$ in this proof. 
	We first represent $u = \frac{1}{t}(ax+by)$ and $v = \frac{1}{t}(bx-ay)$, where $x = \frac{1}{t}(au+bv)$ and $y = \frac{1}{t}(bu-av)$ are two independent Gaussian random variables drawn from $\mathcal{N}(0,1)$. We replace $u,v$ by the new parameterization, 
	\begin{align*}
	\Exp[uv\cdot\relu(au+bv+\xi)^2] &= \Exp\left[\frac{1}{t^2}(ax+by)(bx-ay)\relu(tx+\xi)^2\right] \\
	&= \Exp\left[\frac{1}{t^2} abx^2\relu(tx+\xi)^2\right] -\Exp\left[\frac{1}{t^2} ab\relu(tx+\xi)^2\right]  \\
	&= \Exp\left[\frac{1}{t^2} ab(x^2-1)\relu(tx+\xi)^2\right] 
	\end{align*}
	
	where we used the fact that $\Exp[y] =0$ and $y$ is independent with $x$ and $\xi$. 
	
	Then we expand the expectation by conditioning on $x$ and taking expectation over $\xi$: 
	
	\begin{align*}
	(x^2-1)\Exp[\relu(tx+\xi)^2\mid x] 
	&  = (x^2-1)\int_{-tx}^{\infty} (tx+y)^2\phi(y)dy\\
	&  = (x^2-1)\int_{-tx}^{0} (tx+y)^2\phi(y)dy+ (x^2-1)\int_{0}^{\infty} (tx+y)^2\phi(y)dy\\
	&  = (x^2-1)\int_{0}^{tx} (tx-y)^2\phi(y)dy+ (x^2-1) (C_0t^2x^2+ 2C_1tx + C_2)\\
	& \triangleq H(x) +  (x^2-1) (C_0t^2x^2+ 2C_1tx + C_2)
	\end{align*}
	
	where $C_0 = \int_0^{\infty}\phi(y)dy = \frac{1}{2}$, and $C_1$, $C_2$ are two other constants (the values of which we don't care) that don't depend on $x$. 
	Therefore by Lemma~\ref{lem:H(z)}, we obtain that $|\Exp[H(x)]|\le \tilO(1/\sigma)$ and therefore taking expectation of the equation above we obtain that
	
	\begin{align*}
	\Exp[(x^2-1)\Exp[\relu(tx+\xi)^2\mid x]] 
	%&  = (x^2-1)\int_{-tx}^{\infty} (tx+y)^2\phi(y)dy\\
	%&  = (x^2-1)\int_{-tx}^{0} (tx+y)^2\phi(y)dy+ (x^2-1)\int_{0}^{\infty} (tx+y)^2\phi(y)dy\\
	%&  = (x^2-1)\int_{0}^{tx} (tx-y)^2\phi(y)dy+ (x^2-1) (C_2t^2x^2+ 2C_1tx + C_0)
	& =\Exp[H(x)] +  \Exp[(x^2-1) (C_2t^2x^2+ 2C_1tx + C_0)]\\
	& = 2C_2t^2 \pm \tilO(1/\sigma) = t^2\pm \tilO(1/\sigma)
	\end{align*}
	
	Therefore we have that $\Exp[uv\cdot\relu(au+bv+\xi)^2] = \Exp\left[\frac{1}{t^2} ab(x^2-1)\relu(tx+\xi)^2\right]  = \tilO(1)$. Using the fact that $\Exp[u\relu(au+bv+\xi)]\le \tilO(1)$ and $ \Exp[v\relu(au+bv+\xi)]\le \tilO(1)$, we obtain that 
	
	$\left|\Exp[uv\cdot\relu(au+bv+\xi)^2]  - \Exp[u\relu(au+bv+\xi)]\Exp[v\relu(au+bv+\xi)]\right|=  \tilO(1)$. 
\end{proof}

\begin{lemma}\label{lem:H(z)}
	Suppose $z\sim\mathcal{N}(0,1)$, and let $\phi(x)=\frac{1}{\sigma\sqrt{2\pi}}\exp(-\frac{x^2}{2\sigma^2})$ be the density function of $\mathcal{N}(0,\sigma^2)$ where $\sigma =\Omega(1)$. For $r \le 10\log \sigma$, define $G(z) = \int_{0}^{rz} (rz-y)^2\phi(y)dy$, and $H(z) = (z^2-1)G(z)$. Then we have that $\Exp[|H(z)|]\le \tilO(1/\sigma)$
\end{lemma}
\begin{proof}
	%Essentially we would like to prove that $H(z)$ is close to 0
	Our technique is to approximate $H(z)$ using taylor expansion at point close to 0, and then argue that since $z$ is very unlikely to be very large, so the contribution of large $z$ is negligible. We calculate the derivate of $H$ at point $z$ as follows: 
	\begin{align*}
	H(z)'& = 2zG(z)+ (z^2-1)G'(z) \\
	H(z)'' & = 2G(z) +4zG'(z)+ (z^2-1)G''(z) \\
	H(z)''' & = 6G'(z) + 6zG''(z) + (z^2-1)G'''(z)\\
	%H(z)'''' & = 12G''(z) +  8zG'''(z) + (z^2-1)G''''(z)
	\end{align*}
	Moreover, we have that the derivatives of $G$
	\begin{align*}
	G'(z) & = \int_{0}^{rz}2r(rz-y)\phi(y)dy \\
	G''(z) &= \int_0^{rz}2r^2\phi(y)dy \\
	G'''(z) & = 2r^3\phi(rz) \\
	%G''''(z) & = 2r^4\phi'(rz)
	\end{align*}
	
	Therefore we have that $G'(0) = G''(0) = 0$ and $H'(0) = H''(0) = 0$. Moreover, when $r \le 10\log \sigma$ and $z \le 10\log \sigma$ and we have that bound that $|H'''(z)|\le \tilO(1/\sigma)$. Therefore, we have that for $z\le 10\log \sigma$, $|H(z)|\le \tilO(1/\sigma)$, and therefore we obtain that 
	$\Exp[H(z)\mid |z|\le 10\log \sigma] \Pr[|z|\le 10\log \sigma]\le  \tilO(1/\sigma)$. Since $|H(z)|\le \tilO(1)\cdot z^4$ for any $z$, we obtain that for $z\ge 10\log\sigma$, the contribution is negligible: 	$\Exp[H(z)\mid |z| > 10\log \sigma] \Pr[|z|>  10\log \sigma]\le \tilO(1/\sigma^2)$. Therefore altogether we obtain that $|\Exp[|H(z)|]|\le \tilO(1/\sigma)$. 
\end{proof}


The following two lemmas are not used for the proof of single layer net, though they will be useful for proving the result for 2-layer net. The following lemma bound the correlation between $\check{h}_i$ and $\check{h}_j$. 
\begin{lemma}\label{lem:pairwise-correlation}
	%Under the assumption of Theorem~\ref{thm:single-technical}, 
	Let $\hat{h} = W^Tx$, and $D_h$ satsifies~\eqref{eqn:scaledassumption},   then	for any $i,j$, we have that $|\Exp[\hat{h}_i\hat{h}_j] - \Exp[\hat{h_i}]\Exp[\hat{h_j}]|\le \tilO(1/t)$. 
\end{lemma} 

\begin{proof}
	We expand the definition of $\hat{h}_i$ and $\hat{h}_j$ directly. %The key point is that $\hat{h}_i$ and $\hat{h}_j$ are both linear combination of $x_u$'s,
	\begin{align*}
	\Exp[\hat{h}_i\hat{h}_j] &= \alpha^2 \Exp\left[\left(\sum_{u\in S}W_{ui}x_u\right)\left(\sum_{v\in S}W_{vj}x_v\right)\right]\\	
	&= \alpha^2 \sum_{u\in S}\Exp\left[W_{ui}W_{vi}x_u^2\right]  + \alpha^2\sum_{u\neq v}\Exp\left[W_{ui}W_{vj}x_ux_v\right]\\
	& = \alpha^2 \sum_{u\in S}\Exp\left[W_{ui}W_{vi}x_u^2\right]  + \alpha^2\sum_{u\neq v}\Exp\left[W_{ui}x_u\right]\Exp\left[W_{vj}x_ux_v\right]\\
	& = \alpha^2 \sum_{u\in S}\left(\Exp\left[W_{ui}W_{vi}x_u^2\right] - \Exp[W_{ui}x_u]\Exp[W_{vj}x_v]\right)+ \alpha^2\sum_{u, v}\Exp\left[W_{ui}x_u\right]\Exp\left[W_{vj}x_ux_v\right]\\
	& = \alpha^2 \sum_{u\in S}\left(\Exp\left[W_{ui}W_{vi}x_u^2\right] - \Exp[W_{ui}x_u]\Exp[W_{vj}x_v]\right) + \Exp[\hat{h}_i]\Exp[\hat{h}_j]
	\end{align*}
	where in the third line we use the fact that $W_{ui}x_u$ is independent with $W_{vj}x_v$, and others are basic algebra manipulation. Using Lemma~\ref{lem:pairwise-correlation}, we have that 
	$$\left|\Exp\left[W_{ui}W_{vi}x_u^2\right] - \Exp[W_{ui}x_u]\Exp[W_{vj}x_v]\right|\le \tilO(1)$$
	Therefore we obtain that 
	\begin{align*}
	\left|\Exp[\hat{h}_i\hat{h}_j] - \Exp[\hat{h}_i]\Exp[\hat{h}_j] \right|%&= \alpha^2 \Exp\left[\left(\sum_{u\in S}W_{ui}x_u\right)\left(\sum_{v\in S}W_{vj}x_v\right)\right]\\	
	% &= \alpha^2 \sum_{u\in S}\Exp\left[W_{ui}W_{vi}x_u^2\right]  + \alpha^2\sum_{u\neq v}\Exp\left[W_{ui}W_{vj}x_ux_v\right]\\
	%& = \alpha^2 \sum_{u\in S}\Exp\left[W_{ui}W_{vi}x_u^2\right]  + \alpha^2\sum_{u\neq v}\Exp\left[W_{ui}x_u\right]\Exp\left[W_{vj}x_ux_v\right]\\
	%& = \alpha^2 \sum_{u\in S}\left(\Exp\left[W_{ui}W_{vi}x_u^2\right] - \Exp[W_{ui}x_u]\Exp[W_{vj}x_v]\right)+ \alpha^2\sum_{u, v}\Exp\left[W_{ui}x_u\right]\Exp\left[W_{vj}x_ux_v\right]\\
	& = \alpha^2 \tilO(t) = \tilO(1/t)
	\end{align*}
\end{proof}
The following lemmas shows that the 
\begin{lemma}\label{lem:linearcom}
	Under the single-layer setting of Lemma~\ref{lem:pairwise-correlation}, let $K$ be the support of $h$.  Then for any $k$-dimensional vector $u_K$ such that $|u_K|_{\infty}\le \tilO(1)$, we have that $$\Exp[|u_K^T(\hat{h}_K-\Exp \hat{h}_K)|^2] \le \tilO(k^2/t)$$
	%we have %we have that for any vector 
\end{lemma}
\begin{proof}
	%Finally we consider $u_K^T(\hat{h}_K- \Exp[\hat{h}_K])$: 
	%We bound the expectation of its two norm as follows: 
	We expand our target and obtain, 
	\begin{align*}
	\Exp[|u_K^T(\hat{h}_K-\E \hat{h}_K)|^2]  & = \Exp[|\sum_{i\in K}u_i(\hat{h}_i-\E\hat{h}_i)|^2] \\
	& = \sum_{i\in K}\Exp[u_i^2(h_i-\E\hat{h}_i)^2] + \Exp\left[\sum_{i\neq j} u_iu_j(\hat{h}_i-\E\hat{h}_{i})(\hat{h}_j-\E\hat{h}_{j})\right]\\
	& = \sum_{i\in K}\Exp[(h_i-\E\hat{h}_i)^2]\cdot \tilO(1) + \max_{i\neq j}\{|\Exp[\hat{h}_i\hat{h}_j]-\Exp[\hat{h}_i]\Exp[\hat{h}_j]|\} \cdot \tilO(1) \cdot k^2
	%& \le \beta^2\sum_{i\in K}\Exp[(h_i-\E\hat{h}_i)^2] \cdot \tilO(1)+ \beta^2\max_{i\neq j}\{|\Exp[\hat{h}_i\hat{h}_j\mid \mathcal{E}]-\Exp[\hat{h}_i\mid h]\Exp[\hat{h}_j\mid h]|\} \cdot \tilO(1) \cdot k^2\\
	\end{align*}
	%where we used the fact that conditioned on $\mathcal{E}$, $|u|_{\infty}\le \tilO(1)$.  %and $\mathcal{E}$ is independent 
	By Lemma~\ref{lem:app:var}, we have that $\Exp[(h_i-\E\hat{h}_i)^2]\le \tilO(\|h\|^2/t)$. %By Lemma~\ref{lem:two-correlation}, we obtain that $|\Exp[\hat{h}_i\hat{h}_j\mid h]|\le O(\alpha^2 h_ih_j)$, and by Lemma~\ref{lem:single-reversibility}, we have that $|\Exp[\hat{h}_i\mid h]|\le \alpha h_i +\tilO(\alpha\|h\|/\sqrt{s})\le O(\alpha h_i)$. 
	By Lemma~\ref{lem:pairwise-correlation}, therefore we obtain that $\max_{i\neq j}\{|\Exp[\hat{h}_i\hat{h}_j]-\Exp[\hat{h}_i]\Exp[\hat{h}_j]|\}\le \tilO(1/t) $. Using the fact that $\|h\|^2\le \tilO(k)$,  %and $\beta = 2/k$, we obtain that 
	
	$$	\Exp[|u_K^T(\hat{h}_K-\E\hat{h}_K)|^2] \le \tilO(k^2/t)$$
\end{proof}




==> thm42.tex <==
\begin{theorem}[2-Layer Reversibility and Dropout Robustness]\label{thm:twolayer}
	For $\ell = 2$, and $k_{2} < k_{1} < k_0 < k_2^2$, there exists constant offset vector $b_0, b_1$ such that with probability .9 over the randomness of the weights $(W_0,W_1)$ from prior~\eqref{eqn:multi-prior}, and $h\sim D$ that satisfies~\eqref{eqn:multi-hdistribution}, and observable $x$ generated from the 2-layer generative model described above, the representation obtained from running the network feedforwardly  
	$$\tilde{h}^{(1)} = r(W_0^Tx+b_1), \textrm{ and }\tilde{h}^{(2)} = r(W_1^Th^{(1)}+b_2)$$
	are entry-wise close to the original hidden variables 
	\begin{equation}
	\forall i\in [n_2], \quad \Exp\left[|\tilde{h}_i^{(2)} - h_i^{(2)}|^2\right] \le \tilO(k_2/k_1)\cdot \bar{h}^{(2)}\label{eqn:entry-wise-errorh2}
	\end{equation}
	\begin{equation}
	\forall i\in [n_1], \quad \Exp\left[|\tilde{h}_i^{(1)} - h_i^{(1)}|^2\right] \le \tilO(k_1/k_0)\cdot \bar{h}^{(1)}\label{eqn:entry-wise-errorh1}	
	\end{equation}

where $\bar{h}^{(2) }= \frac{1}{\kappa_{2}}\sum_{i}h^{(2)}_i$ and $\bar{h}^{(1)}= \frac{1}{\kappa_{1}}\sum_{i}h^{(1)}_i$ are the average of the non-zero entries of $h^{(2)}$ and $h^{(1)}$. 

Moreover,  there exists offset vector $b_1'$ and $b_2'$, such that when hidden representation is calculated feedforwardly with dropping out a random subset $G_0$ of size $n_0/2$ in the observable layer and $G_2$ of size $n_1/2$ in the first hidden layer:
$$\tilde{h}^{(1)\drop} = r(2W_0^Tx_{\bar{G_0}}+b_1'), \textrm{ and }\tilde{h}^{(2)} = r(2W_1^Th^{(1)\drop}_{\bar{G_2}}+b_2')$$
are entry-wise close to the original hidden variables in the same form as equation~\eqref{eqn:entry-wise-errorh2} and~\eqref{eqn:entry-wise-errorh1}

\end{theorem}
